Strategic Instrumental Variable Regression: Recovering Causal Relationships From Strategic Responses

In settings where Machine Learning (ML) algorithms automate or inform consequential decisions about people, individual decision subjects are often incentivized to strategically modify their observable attributes to receive more favorable predictions. As a result, the distribution the assessment rule is trained on may differ from the one it operates on in deployment. While such distribution shifts, in general, can hinder accurate predictions, our work identifies a unique opportunity associated with shifts due to strategic responses: We show that we can use strategic responses effectively to recover causal relationships between the observable features and outcomes we wish to predict, even under the presence of unobserved confounding variables. Specifically, our work establishes a novel connection between strategic responses to ML models and instrumental variable (IV) regression by observing that the sequence of deployed models can be viewed as an instrument that affects agents' observable features but does not directly influence their outcomes. We show that our causal recovery method can be utilized to improve decision-making across several important criteria: individual fairness, agent outcomes, and predictive risk. In particular, we show that if decision subjects differ in their ability to modify non-causal attributes, any decision rule deviating from the causal coefficients can lead to (potentially unbounded) individual-level unfairness.

==> algs.tex <==
\section{Risk Minimization and Causal Parameter Recovery}\label{sec:algs}

\subsection{Algorithms}

\iffalse
\begin{algorithm}[H]
\label{alg:cpe}
\SetAlgoLined
\textbf{Input:} $T$\\
 
 Play $T$ uniform random decision rules $\{\vtheta_i\}_{i=1}^T$ where $\vtheta_i^{(j)} \sim_{iid} \text{Unif}(-1,1)$ for each $i$ and $j$\\
 Estimate $\vtheta^*$ via 2SLS: $\widehat{\vtheta} = (\Theta^\top X)^{-1} \Theta^\top \mathbf{y}$\\
 \textbf{return} $\widehat{\vtheta}$\\
 \caption{Causal Parameter Estimation (CPE)}
\end{algorithm}

\begin{algorithm}[H]
\label{alg:ogd}
\SetAlgoLined
\textbf{Input:} $T$, $\{\eta\}_{t=1}^T, \widehat{\vtheta}$\\
 
 \For{$t = 1, 2, ..., T$}{
    $\vtheta_{t+1} = \Pi (\vtheta_{t} - \eta_t \widehat{\Delta}_t(\widehat{\vtheta}, \vtheta_{t}, \vx_{t}, y_{t}))$
 }
$\widehat{\Delta}_t:$ unbiased estimate of $\nabla_{\vtheta_t} f(\vtheta_t)$\\
 \caption{Online Gradient Descent (OGD)}
\end{algorithm}


\begin{algorithm}[H]
\label{alg:full}
\SetAlgoLined
\textbf{Input:} $T_1$, $T_2$, $\boldsymbol{\eta}$\\
 
 $\widehat{\vtheta}_1 =$ CPE$(T_1)$\\
 OGD$(T_2, \{\eta\}_{t=1}^T, \widehat{\vtheta}_1)$\\
 Re-run CPE using all samples collected during CPE and OGD to get final estimate $\widehat{\vtheta}_2$
 
 \textbf{return} $\widehat{\vtheta}_2$\\
 \caption{Combined Risk Minimization and Causal Parameter Recovery}
\end{algorithm}

\subsection{Risk Minimization Derivation}
The loss for playing decision rule $\vtheta_t$ is defined as

\begin{equation} \label{eq:risk}
\begin{aligned}
    f(\vtheta_t) &= \left( \vtheta_t^\top \vx_t(\vtheta_t) - y \right)^2 \\
    &= \left(\vtheta_t^\top \vx_t(\vtheta_t) - \vtheta^{*\top} \vx_t(\vtheta_t) - g(u_t) \right)^2 \\
    &= \left( (\vtheta_t - \vtheta^*)^\top \vx_t(\vtheta_t) - g(u) \right)^2 \\
\end{aligned}
\end{equation}

$\vx_t(\vtheta_t) = \mathbf{z}_t + \Omega \vtheta_t$, where $\Omega = W W^\top$. Substituting this into Equation \ref{eq:risk}, we obtain
\begin{equation}
    f(\vtheta_t) = \left( (\vtheta_t - \vtheta^*)^\top (\mathbf{z}_t + \Omega \vtheta_t) - g(u) \right)^2 
\end{equation}

The gradient of the loss with respect to $\vtheta_t$ is
\begin{equation} \label{eq:true-grad}
\begin{aligned}
    \nabla_{\vtheta_t} f(\vtheta_t) &= \nabla_{\vtheta_t} \left((\vtheta_t - \vtheta^*)^\top (\mathbf{z}_t + \Omega \vtheta_t) - g(u) \right)^2 \\
    &= 2\left( (\vtheta_t - \vtheta^*)^\top (\mathbf{z}_t + \Omega \vtheta_t) - g(u) \right) \left((\mathbf{z}_t + \Omega \vtheta_t) + \Omega^\top (\vtheta_t - \vtheta^*) \right) \\
    &= 2 \left((\vtheta_t - \vtheta^*)^\top \vx_t(\vtheta_t) - g(u) \right) \left(\vx_t(\vtheta_t) + \Omega^\top (\vtheta_t - \vtheta^*) \right) \\
    &= 2 \left(\vtheta_t^\top \vx_t(\vtheta_t) - y \right) \left(\vx_t(\vtheta_t) + \Omega^\top (\vtheta_t - \vtheta^*) \right) \\
\end{aligned}
\end{equation}

\subsection{Regret Analysis}

\iffalse
\begin{equation}
    |\widehat{\vtheta}^* - \vtheta^*| \leq \frac{\sigma_g\sqrt{2nk\log(k/\delta)}}{|\sum_{i=1}^T (\vtheta_i - \Bar{\vtheta})(x_i - \Bar{x})|}
\end{equation}
\fi 

\subsubsection{Regret due to Algorithm \ref{alg:cpe}}
\begin{definition} (Regret)
The regret of \Cref{alg:full} is 
\begin{equation*}
    R(T) = T f(\vtheta^*) - \sum_{i = 1}^T f(\vtheta_t)
\end{equation*}
\end{definition}

$O(T_1)$


\subsubsection{Bounding $\| \widehat{\vtheta} - \vtheta^* \|_2$} \label{sec:theta}
Recall that $\widehat{\vtheta} = (\Theta^\top X)^{-1} \Theta^\top \mathbf{y}$. Plugging this into $\| \widehat{\vtheta} - \vtheta^* \|_2$, we get
\begin{equation}
   \| \widehat{\vtheta} - \vtheta^* \|_2 = \| (\Theta^\top X)^{-1} \Theta^\top \mathbf{y} - \vtheta^* \|_2
\end{equation}

Next, we substitute in our expression for $\mathbf{y}$:
\begin{equation} \label{eq:bound1}
\begin{aligned}
   \| \widehat{\vtheta} - \vtheta^* \|_2 
   &= \| (\Theta^\top X)^{-1} \Theta^\top (X \vtheta^* + \mathbf{g}) - \vtheta^* \|_2\\
   &= \| (\Theta^\top X)^{-1} \Theta^\top X \vtheta^* + (\Theta^\top X)^{-1} \Theta^\top \mathbf{g} - \vtheta^* \|_2\\
   &= \| \vtheta^* + (\Theta^\top X)^{-1} \Theta^\top \mathbf{g} - \vtheta^* \|_2\\
   &= \| (\Theta^\top X)^{-1} \Theta^\top \mathbf{g} \|_2\\
   & \leq \| (\Theta^\top X)^{-1} \|_2 \| \Theta^\top \mathbf{g} \|_2\\
   & \leq \frac{\| \Theta^\top \mathbf{g} \|_2}{\sigma_{min}(\Theta^\top X)}
\end{aligned}
\end{equation}


Focusing on the numerator, note that 
\begin{equation}
    \| \Theta^\top \mathbf{g} \|_2 = \sqrt{\sum_{j=1}^m \left(\sum_{i=1}^n \theta_i^{(j)} g(u_i) \right)^2}
\end{equation}
Since $g(u_i)$ is a zero-mean sub-Gaussian random variable with variance parameter $\sigma_g$ and for each $j$, the $j$th entry of $\theta_i$, denoted $\theta_i^{(j)}$, is drawn uniformly from $\{\frac{-1}{\sqrt{m}}, \frac{1}{\sqrt{m}} \}$ (with variance $1/4$), thus for any $i$, the product $\theta_i^{(j)} g(u_i)$ will also be a sub-Gaussian random variable. Because $\theta_i^{(j)}$ and $g(u_i)$ are zero-mean and $g(u_i)$ is independent from $\theta_i^{(j)}$ for all $j$, the variance of $\theta_i^{(j)} g(u_i)$ is $\sigma_g^2/4$. In order to bound $\sum_{i=1}^n \theta_i^{(j)} g(u_i)$ with high probability, we make use of the following lemma:

\begin{lemma}[High probability bound on the sum of unbounded sub-Gaussian random variables] \label{lemma:chernoff}
Let $x_i \sim \text{subG}(0, \sigma^2)$. For any $\delta \in (0, 1)$, with probability at least $1 - \delta$,
\begin{equation}
    \Big|\sum_{i=1}^n x_i\Big| \leq \sigma \sqrt{2n\log(1/\delta)}
\end{equation}
\end{lemma}

Applying Lemma \ref{lemma:chernoff}, we get
\begin{align*}
    \left \| \Theta^\top \mathbf{g} \right \|_2 
    &\leq \sqrt{\sum_{j=1}^m \left(\sigma_g \sqrt{(1/2)n\log(1/\delta_j)} \right)^2}\\
    &\leq \sqrt{\sum_{j=1}^m \sigma_g^2 (1/2)n\log(m/\delta)} \tag{by a union bound, where $\delta_j=\delta/m$ for all $j$}\\
    &\leq \sigma_g \sqrt{(1/2)nm\log(m/\delta)}\\
\end{align*}
with probability at least $1 - \delta$. Substituting this back into Equation \ref{eq:bound1}, we get
\begin{equation}
    \| \widehat{\vtheta} - \vtheta^* \|_2 \leq \frac{\sigma_g \sqrt{(1/2)nm\log(m/\delta)}}{\sigma_{min}(\Theta^\top X)}
\end{equation}
with probability at least $1 - \delta$. Next we bound the denominator, $\sigma_{min}(\Theta^\top X)$.
\fi
\begin{equation}
    \begin{aligned}
        \sigma_{min}(\Theta^\top X) 
        &= \sigma_{min}(\sum_{i=1}^n \vx_i \vtheta_i^\top)\\
        &= \sigma_{min}(\sum_{i=1}^n \vz_i \vtheta_i^\top + WW^\top \vtheta_i \vtheta_i^\top)\\
        &= \sigma_{min}(A + B),
    \end{aligned}
\end{equation}
where $A = \sum_{i=1}^n \vz_i \vtheta_i^\top$ and $B = \sum_{i=1}^n WW^\top \vtheta_i \vtheta_i^\top$. By definition, 

\begin{equation}
    \sigma_{min}(A+B) = \min_{\va, \|\va\|_2 = 1} \|(A + B)\va\|_2.
\end{equation}

By the triangle inequality, 
\begin{equation} \label{eq:triangle}
\begin{aligned}
    \sigma_{min}(A+B) 
    &\geq \min_{\va, \|\va\|_2 = 1} \left( \|B\va\|_2 - \|A\va\|_2 \right)\\
    &\geq \min_{\va, \|\va\|_2 = 1} \|B\va\|_2 - \|A\|_2\\
    &\geq \sigma_{min}(B) - \|A\|_2\\.
\end{aligned}
\end{equation}

We start by bounding $\|A\|_2$.

\begin{lemma}[Matrix Bernstein]\cite{tropp2015introduction} \label{lemma:bernstein}
    Consider a finite sequence $\{S_i\}_{i=1}^n$ of independent, random matrices with common dimension $d_1 \times d_2$. Assume that $\mathbb{E}[S_i] = 0_{d_1 \times d_2}$ and $\|S_i\|_2 \leq L$ for each index $i$.
    
    Introduce the random matrix $A = \sum_{i=1}^n S_i$. Let $v(A)$ be the matrix variance statistic of the sum:
    \begin{equation*}
        \begin{aligned}
            v(A) 
            &= \max\left\{ \left\|\mathbb{E}[AA^\top]\|_2, \|\mathbb{E}[A^\top A] \right\|_2 \right\}\\
            &= \max\left\{ \left\| \sum_{i=1}^n \mathbb{E}[S_i S_i^\top]\|_2, \| \sum_{i=1}^n \mathbb{E}[S_i S_i^\top] \right\|_2 \right\}.
        \end{aligned}
    \end{equation*}
Then for all $t \geq 0$,
\begin{equation*}
    P(\|A\|_2 \geq t) \leq (d_1 + d_2) \exp \left( \frac{-t^2/2}{v(A) + Lt/3} \right)
\end{equation*}
\end{lemma}

Let $S_i = \vz_i \vtheta_i^\top$. $\|\mathbb{E}[S_i]\| = 0$, since $\mathbb{E}[\vtheta_i] = \mathbf{0}$, and $\vtheta_i$ is independent from $\vz_i$.

\begin{equation*}
\begin{aligned}
    v(A) 
    &= \max\left\{ \left\| \sum_{i=1}^n \mathbb{E}[S_i S_i^\top]\|_2, \| \sum_{i=1}^n \mathbb{E}[S_i S_i^\top] \right\|_2 \right\}\\
    &\leq n\max\left\{ \left\|\mathbb{E}[S_i S_i^\top]\|_2, \| \mathbb{E}[S_i S_i^\top] \right\|_2 \right\}\\
    &\leq n
\end{aligned}
\end{equation*}

$\|S_i\|_2 \leq \sqrt{m}$, so $L = \sqrt{m}$.

Applying Lemma \ref{lemma:bernstein}, we obtain

\begin{equation}
    P(\|A\|_2 \geq t) \leq 2m \exp \left( \frac{-t^2/2}{n + \sqrt{m}t/3} \right)
\end{equation}

By setting the RHS equal to $\delta$ and rearranging terms, we get 
\begin{equation}
    \|A\|_2 \leq \sqrt{2n \log \left(\frac{2m}{\delta}\right)}
\end{equation}
with probability at least $1 - \delta$.

Plugging this into Equation \ref{eq:triangle}, we get
\begin{equation} \label{eq:triangle-A}
    \sigma_{min}(A+B) \geq \sigma_{min}(B) - \sqrt{2n \log \left(\frac{2m}{\delta}\right)}.
\end{equation}

Next we bound $\sigma_{min}(B)$.

\begin{equation}
    \begin{aligned}
        \sigma_{min}(B) 
        &= \sigma_{min}(WW^\top \sum_{i=1}^n \vtheta_i \vtheta_i^\top)\\
        &\geq \sigma_{min}(WW^\top) \sigma_{min}(\sum_{i=1}^n \vtheta_i \vtheta_i^\top)
    \end{aligned}
\end{equation}

Since $WW^\top$ and $\sum_{i=1}^n \vtheta_i \vtheta_i^\top$ are both symmetric matrices with non-negative eigenvalues, $\sigma_{min}(WW^\top) = \lambda_{min}(WW^\top)$ and $\sigma_{min}(\sum_{i=1}^n \vtheta_i \vtheta_i^\top) = \lambda_{min}(\sum_{i=1}^n \vtheta_i \vtheta_i^\top)$. $\lambda_{min}(WW^\top) \geq 1$ by assumption, so 
\begin{equation}
    \sigma_{min}(B) \geq \lambda_{min}(\sum_{i=1}^n \vtheta_i \vtheta_i^\top).
\end{equation}

We now use the Matrix Chernoff bound to get a lower bound for $\lambda_{min}(\sum_{i=1}^n \vtheta_i \vtheta_i^\top)$.


\iffalse
\subsubsection{Bounding $\| \Delta_t - \widehat{\Delta}_t \|_2$}

Loss function (Equation \ref{eq:risk}):
\begin{equation}
    f(\vtheta_t) = (\vtheta_t^\top \vx_t - y_t)^2
\end{equation}


True Derivative (Equation \ref{eq:true-grad}):
\begin{equation}
    \Delta_t = \nabla_{\vtheta_t} f(\vtheta_t) = 2(\vtheta_t^\top \vx_t - y_t)(\vx_t + \Omega^\top (\vtheta_t - \vtheta^*))
\end{equation}

Estimate of Derivative:
\begin{equation}
    \widehat{\Delta}_t = \widehat{\nabla_{\vtheta_t} f(\vtheta_t)} = 2(\vtheta_t^\top \vx_t - y_t)(\vx_t + \Omega^\top (\vtheta_t - \widehat{\vtheta}))
\end{equation}

Bound on Estimate:
\begin{equation}
\begin{aligned}
    \| \Delta_t - \widehat{\Delta}_t \|_2 
    &= 2\left \| \left(\vtheta_t^\top \vx_t - y_t \right) \left(\vx_t + \Omega^\top (\vtheta_t - \vtheta^*) \right) - \left(\vtheta_t^\top \vx_t - y_t \right) \left(\vx_t + \Omega^\top (\vtheta_t - \widehat{\vtheta}) \right) \right \|_2 \\
    &= 2\left\| \left(\vtheta_t^\top \vx_t - y_t \right) \Omega^\top \left(\widehat{\vtheta} - \vtheta^* \right) \right \|_2 \\
    &\leq 2\left \| (\vtheta_t^\top \vx_t - y_t) \Omega^\top \right \| \left \| \widehat{\vtheta} - \vtheta^* \right \|_2
\end{aligned}
\end{equation}


\subsubsection{Regret due to Algorithm \ref{alg:ogd}}
Next we use our bound for $\| \Delta_t - \widehat{\Delta}_t \|_2$ to bound the regret achieved by Algorithm \ref{alg:ogd}. Let $\vtheta^R$ denote the optimal $\vtheta$ parameter for risk minimization. Note that $\vtheta^R$ does not necessarily equal $\vtheta^*$. If the loss function $f$ is convex, then 
\begin{equation}
\begin{aligned}
    f(\vtheta_t) - f(\vtheta^R) &\leq \Delta_t^\top (\vtheta_t - \vtheta^R) \\
    &= (\widehat{\Delta}_t + \Delta_t - \widehat{\Delta}_t)^\top (\vtheta_t - \vtheta^R) \\
    &= \widehat{\Delta}_t^\top (\vtheta_t - \vtheta^R) + (\Delta_t - \widehat{\Delta}_t)^\top (\vtheta_t - \vtheta^R)
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
    \|\vtheta_{t+1} - \vtheta^R\|^2 &= \| \Pi(\vtheta_t - \eta_t \widehat{\Delta}_t) - \vtheta^R \|^2_2 \\
    &\leq \| \vtheta_t - \eta_t \widehat{\Delta}_t - \vtheta^R \|^2_2 \\
    &= \|\vtheta_t - \vtheta^R \|^2_2 + \eta_t^2 \|\widehat{\Delta}_t \|^2_2 - 2\eta_t \widehat{\Delta}_t^\top (\vtheta_t - \vtheta^R)
\end{aligned}
\end{equation}

\begin{equation}
    \widehat{\Delta}_t^\top (\vtheta_t - \vtheta^R) \leq \frac{\|\vtheta_t - \vtheta^R \|^2_2 - \|\vtheta_{t+1} - \vtheta^R\|^2_2}{2\eta_t} + \frac{1}{2} \eta_t \|\widehat{\Delta}_t \|^2_2
\end{equation}

Plugging this into our expression for $f(\vtheta_t) - f(\vtheta^R)$, we obtain
\begin{equation}
    f(\vtheta_t) - f(\vtheta^R) \leq \frac{\|\vtheta_t - \vtheta^R \|^2_2 - \|\vtheta_{t+1} - \vtheta^R\|^2_2}{2\eta_t} + \frac{1}{2} \eta_t \|\widehat{\Delta}_t \|^2_2 + (\Delta_t - \widehat{\Delta}_t)^\top (\vtheta_t - \vtheta^R)
\end{equation}

Let $\widehat{G} = \max_t \|\widehat{\nabla}_t \|_2$, $D = \max_t \| \vtheta_t - \vtheta^R \|^2_2$, $C = 2\max_t \|(\vtheta_t^\top \vx_t - y_t) \Omega^\top \|_2$, and define $\frac{1}{\eta_0} = 0$. Then,
\begin{equation}
\begin{aligned}
    \sum_{t=1}^{T_2} f(\vtheta_t) - f(\vtheta^R) &\leq \sum_{t=1}^{T_2} \frac{\|\vtheta_t - \vtheta^R \|^2_2 - \|\vtheta_{t+1} - \vtheta^R\|^2}{2\eta_t} + \frac{1}{2} \eta_t \widehat{G}^2 + (\Delta_t - \widehat{\Delta}_t)^\top (\vtheta_t - \vtheta^R) \\
    &\leq \frac{1}{2} \sum_{t=1}^{T_2} \|\vtheta_t - \vtheta^R \|^2 (\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}}) + \frac{1}{2} \widehat{G}^2 \sum_{t=1}^{T_2} \eta_t  + \sum_{t=1}^{T_2} (\Delta_t - \widehat{\Delta}_t)^\top (\vtheta_t - \vtheta^R) \\
    &\leq \frac{1}{2} D^2 \frac{1}{\eta_T} + \frac{1}{2} \widehat{G}^2 \sum_{t=1}^{T_2} \eta_t  + \sum_{t=1}^{T_2} (\Delta_t - \widehat{\Delta}_t)^\top (\vtheta_t - \vtheta^R) \\
    &\leq \frac{1}{2} D^2 \frac{1}{\eta_T} + \frac{1}{2} \widehat{G}^2 \sum_{t=1}^{T_2} \eta_t + \sum_{t=1}^{T_2} \|(\Delta_t - \widehat{\Delta}_t)^\top (\vtheta_t - \vtheta^R) \|_2 \\
    &\leq \frac{1}{2} D^2 \frac{1}{\eta_T} + \frac{1}{2} \widehat{G}^2 \sum_{t=1}^{T_2} \eta_t + \sum_{t=1}^{T_2} \|\Delta_t - \widehat{\Delta}_t \|_2 \| \vtheta_t - \vtheta^R \|_2 \\
    &\leq \frac{1}{2} D^2 \frac{1}{\eta_T} + \frac{1}{2} \widehat{G}^2 \sum_{t=1}^{T_2} \eta_t + D \max_t  \|\Delta_t - \widehat{\Delta}_t \|_2  T_2 \\
    &\leq \frac{1}{2} D^2 \frac{1}{\eta_T} + \frac{1}{2} \widehat{G}^2 \sum_{t=1}^{T_2} \eta_t + CD \| \widehat{\vtheta} - \vtheta^* \|_2 T_2 \\
\end{aligned}
\end{equation}

\khcomment{In the traditional setting, pick $\eta_t = \frac{G}{D \sqrt{t}}$}

\subsubsection{Regret due to Algorithm \ref{alg:full}}
\begin{equation}
    R(T) \leq C_1 T_1 + \frac{1}{2} D^2 \frac{1}{\eta_T} + \frac{1}{2} \widehat{G}^2 \sum_{t=1}^{T_2} \eta_t + C_2 D \| \widehat{\vtheta} - \vtheta^* \|_2 T_2
\end{equation}
\fi

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} See Conclusion.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} No immediate negative societal impacts come to mind.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} See Appendix.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} We included links to the publicly available datasets we begin with. See \Cref{sec:experiment} for an abridged description of how we modify this data and run our methods. See \Cref{sec:omitted-experiments} for a full description.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See \Cref{sec:omitted-experiments} for all training details and justifications for how they were chosen.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} See \Cref{fig:estimation_error,fig:ols-2sls-estimates,fig:credit-estimation_error,fig:credit-outcome} for all estimates with error bars (after 10 runs with different random seeds).
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} See Appendix \ref{sec:answers}.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} See \Cref{sec:experiment}
  \item Did you mention the license of the assets?
    \answerYes{} We cite the creators or authors of the two datasets we use and link to where they can be publicly accessed. See Appendix \ref{sec:answers}.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{} We do not provide any new assets. We use publicly-accessed data and provide code for modifying it before applying our methods. 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{} See Appendix \ref{sec:answers}.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{} See Appendix \ref{sec:answers}.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> disparate_effects.tex <==
\section{The Disparate Effects of Using Non-Causal Assessments}\label{sec:fairness}
While making predictions based on causal relationships is important from an ML perspective for reasons of generalization and robustness, the societal implications of using non-causal relationships to make decisions are perhaps an even more persuasive reason to use causally-relevant attributes when making predictions in consequential domains. In particular, it could be the case that a certain portion of the population is worse at strategically manipulating features which are not causally relevant than the rest of the population. If non-causally relevant attributes are used in the decision-making process, these individuals will be unfairly seen by the decision-maker as less qualified than their peers, even if their initial features and ability for improvement are the same. 

\xhdr{Disparity Between Agents.} A basic desideratum for fairness in our setting is that two individual decision-subjects with the same \khedit{outcome $y$ for any deployed assessment rule $\vtheta$} should receive similar predictions. As we will illustrate in the following example, this is the case if the assessment rule $\vtheta$ used to make predictions is equal to $\vtheta^*$. Throughout this section we use $\mathcal{C} \subseteq \{1, \ldots, n\}$ to denote the indices of observable features $\vx$ which are causally relevant (i.e., $\theta^*_i > 0$ for $i \in \mathcal{C}$) to outcomes $y$.

\khedit{Consider the problem of assigning predictions to two agents $\vu$ and $\vu'$ with attributes $\vb = \vb'$, $o = o'$, and $(\mathcal{E}\mathcal{E}^\top)_{ij} = (\mathcal{E}'\mathcal{E}'^\top)_{ij}$ if $i \in \mathcal{C}$ or $j \in \mathcal{C}$. Otherwise, $(\mathcal{E}\mathcal{E}^\top)_{ij} \geq (\mathcal{E}'\mathcal{E}'^\top)_{ij}$ with equality holding for at least one $(i,j)$ pair. Intuitively, this corresponds to a setting in which the initial observable features and mapping between the deployed assessment rule $\vtheta$ and changes in causally-relevant observable features $\vx_\mathcal{C}$ are the same for each agent, but one agent is better at manipulating non-causally relevant observable features than the other. Under such a setting, $y = y'$ no matter what assessment rule is used to make predictions, and $\hat{y} = \hat{y}'$ if $\vtheta = \vtheta^*$. On the other hand, if $\vtheta \neq \vtheta^*$, $\hat{y} \geq \hat{y}'$ even though $y = y'$!. Moreover, the difference between $\hat{y}$ and $\hat{y'}$ grows with how much better agent $\vu$ is compared to $\vu'$ at manipulating features which are not causally relevant, the number of features which are not causally relevant, the number of actions available to the agents, and the weight that the assessment rule $\vtheta$ places on non-causally relevant attributes. Formally, we lower-bound this difference as follows.

\begin{proposition}\label{thm:nec}
The gap in predictions can be bounded as
\small
\begin{equation*}
\begin{aligned}
    &\hat{y}_1 - \hat{y}_2 \geq d \delta (n - n_C)^2 \epsilon^2 
\end{aligned}
\end{equation*}
\normalsize
if $\vtheta^* \succcurlyeq \mathbf{0}_m$, where $n$ is the number of observable features, $n_C$ is the number of causally relevant observable features, $d$ is the number of actions each agent can invest effort in, $\delta = \min_{i \not\in \mathcal{C}, j \not\in \mathcal{C}, k \in \{1, \ldots, d\}} \mathcal{E}_{ik} \mathcal{E}_{jk} - \mathcal{E}'_{ik} \mathcal{E}'_{jk}$, and $\epsilon = \min_{i \not\in \mathcal{C}} \theta_i$ is the minimum weight $\vtheta$ places on observable features which are not causally relevant.
\end{proposition}
}

See Appendix  \ref{sec:nec-derivations} for full derivations, which follow from straightforward algebraic manipulation.

\iffalse
\xhdr{Disparity Between subpopulations.} An analogous bound holds when different \emph{subpopulations} of agents differ only in non-causal ways. In order to see how using non-causal relationships to make predictions may lead to inequality across different subpopulations, consider the following example, which is an extension of the previous example to the population setting.



Consider the setting in which the agent population consists of two different subpopulations: an ``advantaged group'' $A$ which is better at manipulating features which are not causally relevant than a ``disadvantaged group'' $D$. Intuitively, this difference in ability to manipulate  features which are not causally relevant should have no impact on the expected predicted outcome, as both populations have equal ability when it comes to altering their causally-relevant attributes. \khedit{In particular, we study the setting in which $\E_A[o] = \E_D[o]$, $\E_A[\vb] = \E_D[\vb]$, $\E_A[\mathcal{E}\mathcal{E}^\top]_{ij} = \E_D[\mathcal{E}\mathcal{E}^\top]_{ij}$ for $i$ or $j \in \mathcal{C}$, and $\E_A[\mathcal{E}\mathcal{E}^\top]_{ij} \geq \E_D[\mathcal{E}\mathcal{E}^\top]_{ij}$ for $i,j \not \in \mathcal{C}$. Note that in this setting, $\E_A[y] = \E_D[y]$ always, but the expected prediction for both subpopulations need not be the same. Formally, we can lower-bound the difference between $\mathbb{E}_A[\hat{y}]$ and $\mathbb{E}_D[\hat{y}]$ as follows:

\begin{proposition}
The gap in expected prediction between subpopulations $A$ and $D$ is at least 
\small
\begin{equation*}
\begin{aligned}
    &\E_A[\hat{y}] - \E_D[\hat{y}] \geq d \delta (n - n_C)^2 \epsilon^2    
\end{aligned}
\end{equation*}
\normalsize
if $\vtheta^* \succcurlyeq \mathbf{0}_m$, where $n$ is the number of observable features, $n_C$ is the number of causally-relevant observable features, $d$ is the number of actions each agent can invest effort in, $\delta = \min_{i \not\in \mathcal{C}, j \not\in \mathcal{C}, k \in \{1, \ldots, d\}} \E_A[\mathcal{E}_{ik}\mathcal{E}_{jk}] - \E_D[\mathcal{E}_{ik}\mathcal{E}_{jk}]$, and $\epsilon = \min_{i \not\in \mathcal{C}} \theta_i$ is the minimum weight $\vtheta$ places on observable features which are not causally relevant.
\end{proposition}
}
Much like the bound in Lemma \ref{thm:nec}, the bound on $\E_A[\hat{y}] - \E_D[\hat{y}]$ will never be negative, and will grow with the gap in ability between $A$ and $D$ to manipulate features which are not causally relevant, the number of such features, the number of actions available to the agents, and the weight that $\vtheta$ places on attributes which are not causally relevant. The derivation is analogous to the derivation of Lemma \ref{thm:nec}. 
\fi 

We also note that if causal relationships are used to make predictions (i.e., if $\vtheta = \vtheta^*$), statistical parity is satisfied between subpopulations which differ only in their ability to manipulate attributes which are not causally relevant.

\begin{definition}[Statistical Parity]
A predictor $\vtheta$ is said to satisfy statistical parity for two subpopulations $G$ and $G'$ if 
\small
\begin{equation*}
    \mathbb{P}_G(\widehat{y} \leq t) = \mathbb{P}_{G'}(\widehat{y} \leq t), \forall t.
\end{equation*}
\normalsize
\end{definition}

\begin{proposition}
If the joint distribution over $\vb$, $o$, and $[\mathcal{E}\mathcal{E}^\top]_{ij}$ ($i$ or $j \in \mathcal{C}$) is the same for subpopulations $G$ and $G'$, then statistical parity between $G$ and $G'$ is satisfied if $\vtheta = \vtheta^*$.
\end{proposition}

See Appendix \ref{sec:statistical-parity} for the proof, which follows straightforwardly from algebraic manipulation. 


\iffalse
\subsection{The Effects of Overestimation on Different Subpopulations}
Another way to characterize the (un-)fairness of a deployed decision rule $\vtheta$ is to compare the expected amount of over/under-estimation of an agent's outcome across different agent subpopulations. To formalize this notion of fairness, we make use of the notion of an \emph{overestimation gap} between the expected outcome and expected predicted outcome.
\begin{definition}[Overestimation Gap]
For a given subpopulation $G$, define the overestimation gap between the expected outcome and expected predicted outcome as $\E_G[\hat{y}_t - y_t]$. Moreover, define the \emph{difference in overestimation gap} between any two subpopulations $G$ and $G'$ as 
\begin{equation*}
    \Delta(G,G') = \E_G[\hat{y}_t - y_t] - \E_{G'}[\hat{y}_t - y_t].
\end{equation*}
\end{definition}

In order to illustrate the potential differences in overestimation gap that $\vtheta \neq \vtheta^*$ may cause, we return to the setting introduced in Example \ref{ex:2}.

\begin{example}[Example \ref{ex:2}, continued]
Under this setting, we can bound the difference in overestimation gap as follows:

\begin{theorem}\label{thm:dif-in-pred-gap}
If the principal uses a decision rule $\vtheta \neq \vtheta^*$ to make predictions, then
\begin{equation*}
    \Delta(A,D) = \Omega((n - n_{\mathcal{C}})n_{\mathcal{C}} d \gamma_1 (2\gamma_2 - \gamma_3) + (n - n_{\mathcal{C}})^2 d \gamma_1^2),
\end{equation*}
where $n$ is the number of observable features, $n_\mathcal{C}$ is the number of causal observable features, $d$ is the number of actions each agent can invest effort in, and $\gamma_1, \gamma_2, \gamma_3$ are positive, instance-dependent constants. 
\end{theorem}

See Appendix \ref{sec:pred-gap-derivations} for the full derivations. Note that in some special cases (namely when $\gamma_2 << \gamma_3$), the difference in overestimation gap can actually be negative. Intuitively, this can occur whenever $\vtheta$ induces the advantaged decision-subjects to invest efforts which greatly improve their true outcome, but only slightly improve their predicted outcome when compared to the effort investments made by the disadvantaged population. For more details, see Appendix \ref{sec:neg-pred-gap}.

While it is possible for the difference in overestimation gap to be negative under certain special settings, it is important to note that the statistical parity gap and difference between $\E_A[y]$ and $\E_D[y]$ are always positive, even when the difference in overestimation gap is negative. Additionally, this difference is strictly non-negative under many common situations. In particular, the difference in overestimation gap for two subpopulations is non-negative whenever $\vtheta$ \emph{overestimates} the causal effects of observable features (i.e., $\vtheta = \vtheta^* + \boldsymbol{\epsilon}$, $\boldsymbol{\epsilon} \succcurlyeq 0$), or whenever $\vtheta$ \emph{underestimates} the causal effects, but the amount of underestimation is bounded below some threshold. The proofs of the following two corollaries follow straightforwardly from the derivation of Theorem \ref{thm:dif-in-pred-gap}.

\begin{corollary}\label{cor:1}
If $\vtheta = \vtheta^* + \boldsymbol{\epsilon}$ ($\boldsymbol{\epsilon} \succcurlyeq 0$), the difference in overestimation gap is strictly non-negative and is lower-bounded as $\Delta(A,D) \geq \Omega((n - n_\mathcal{C})^2 d \gamma_1^2)$.
\end{corollary}

\begin{corollary}\label{cor:2}
If $\vtheta \geq \frac{1}{2} \vtheta^*$, the difference in overestimation gap is strictly non-negative and is lower-bounded as $\Delta(A,D) \geq \Omega((n - n_\mathcal{C})^2 d \gamma_1^2)$.
\end{corollary}

\end{example}
\fi 

==> estimation-bound.tex <==
\section{Finite Sample IV Estimate Bound for General Setting}
\subsection{Model}
We present our model as a system of linear equations expressed as such
\begin{equation}
    \begin{cases}
    y_i = \mb x^\top \mb \theta^* + g(u_i)\\
    \mb x_i = \mb z_t + WW^\top \mb\theta_i = \mb z_t + \Omega \mb\theta_i 
    \end{cases}
\end{equation}
where $g(u_i)\in\RR^k$ is a mean-zero sub-Gaussian random variable with variance parameter $\sigma_g$.
Now, we can rewrite the reward $y_i$ as 
\begin{align*}
    y_i &= (\mb z_t + WW^\top \mb\theta_i)^\top \mb\theta^* + g(u_i)\\
    &= \mb\theta_i^\top WW^\top \mb\theta^* + \mb z_t\top \mb\theta^* + g(u_i)\\
    &= \mb\theta_i^\top \Gamma + \mb z_t\top \mb\theta^* + g(u_i), \tag{where $\Gamma = WW^\top \mb\theta^*$}
\end{align*}

\subsection{Finite Sample Analysis}

\begin{restatable}[Treatment effect approximation bound for General Model]{theorem}{generaltreatmentapproximationbound}\label{thm:general-treatment-approximation-bound}


Let $\theta_1,\dots,\theta_n\in[0,1]^k$ be a sequence of instruments. Suppose there is a sequence of $n$ agents such that each agent $i$ has private type $u_i$ drawn independently from $\cU$, plays features $x_i$ under instrument $\theta_i$, and receives reward $y_i$. Let sample set $S=(x_i,y_i,\theta_i)_{i=1}^n$. For any $\delta\in(0,1)$, the difference between the true causal effect $\theta^*$ and its IV estimate $\hat{\theta}_S^*$ based on sample set $S$ satisfies the following approximation bound $A(S,\delta)$:
    \[\norm{\hat{\theta}_S^*-\theta^*}_2 \leq A(S,\delta) := \frac{\sigma_g\sqrt{2nk\log(k/\delta)}}{\sigma_{\min}\left\{\sum_{i=1}^n x_i\theta_i^{\intercal}\right\}},\]
where $\sigma_{\min}\{\cdot\}$ denotes the smallest singular value.
\end{restatable}

\begin{proof}
    See \cref{sec:general-approximation-bound-proof} for a proof.
\end{proof}


\subsection{Finite Sample Analysis Proof}
\label{sec:general-approximation-bound-proof}
Given $n \in \RR$ samples $\left\{(\theta_i, x_i, y_i)\right\}_{i=1}^n$, of the revealed treatment effect $\theta_i$, chosen features $x_i$, and reward $y_i$ at each round $i$, we would like to bound the difference between the predicted exogenous treatment effect, denoted $\hat{\theta}_S^*$, and the true treatment effect $\theta^*$.

\subsubsection{IV Estimate}
First, we form the estimate $\hat{\theta}_S^*$ of $\theta$ via Two-Stage Least Squares (2SLS) regression. In the first stage, we form the OLS estimate $\hat{\Gamma}_S$ of $\Gamma$ by regressing $y_i$ onto $\theta_i$ and the OLS estimate $\hat{\omega}_S$ of $\omega$ by regressing $x_i$ onto $\theta_i$:
\begin{equation}
    \hat{\Gamma}_S = \bigg(\sum_{i=1}^n\theta_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_iy_i
    \hspace{.4cm}
    \text{ and }
    \hspace{.4cm}
    \hat{\omega}_S = \bigg(\sum_{i=1}^n\theta_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_ix_i^\intercal
\end{equation}

Second, we take the inverse of $\hat{\Gamma}_S$ times $\hat{\omega}_S$ as the predicted causal effect vector $\hat{\theta}_S^*$:
\begin{align*}
    \hat{\theta}_S^*
    &= (\hat{\omega}_S^\intercal)^{-1}\hat{\Gamma}_S\\
    &= \left(\bigg(\sum_{i=1}^n\theta_ix_i^\intercal\bigg)^{-1}\right)^\intercal\bigg(\sum_{i=1}^n\theta_i\theta_i^\intercal\bigg)^\intercal\bigg(\sum_{i=1}^n\theta_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_iy_i\\
    &= \bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\bigg(\sum_{i=1}^n\theta_i\theta_i^\intercal\bigg)\bigg(\sum_{i=1}^n\theta_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_iy_i\\
    &= \bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_iy_i
\end{align*}

Finally, we take the norm of the difference between $\theta^*$ and IV estimate $\hat{\theta}_S^*$
\begin{align*}
    \norm{\hat{\theta}_S^* - \theta^*}_2 &= \norm{\bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_i(\theta^*^\intercal x_i + g(u_i))^\intercal}_2\\
    &= \norm{\bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\bigg(\sum_{i=1}^n\theta_i(\theta^*^\intercal x_i)^\intercal + \sum_{i=1}^n\theta_ig(u_i)\bigg)}_2\\
    &= \norm{\bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\bigg(\sum_{i=1}^n\theta_ix_i^\intercal\theta^* + \sum_{i=1}^n\theta_ig(u_i)\bigg)}_2\\
    &= \norm{\bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)\theta^* + \bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_ig(u_i)}_2\\
    &= \norm{\theta^* + \bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_ig(u_i)}_2\\
    &= \norm{\bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}\sum_{i=1}^n\theta_ig(u_i)}_2\\
    &\leq \norm{\bigg(\sum_{i=1}^nx_i\theta_i^\intercal\bigg)^{-1}}_2\norm{\sum_{i=1}^n\theta_ig(u_i)}_2\tag{by Cauchy-Schwarz}\\
    &= \frac{\norm{\sum_{i=1}^n\theta_ig(u_i)}_2}{\sigma_{\min}\bigg\{\sum_{i=1}^nx_i\theta_i^\intercal\bigg\}},\\
\end{align*}
where $\sigma_{\min}\{\cdot\}$ denotes the minimum singular value.

Now, we upper bound the numerator of the last line above in the following \Cref{eq:general-approximation-bound-numerator}:
\begin{lemma}\label{eq:general-approximation-bound-numerator}
For any $\delta \in (0,1)$, with probability at least $1-\delta$, the numerator of the approximation bound $A(S,\delta)$ given in \Cref{thm:general-treatment-approximation-bound} is 
\begin{equation}
    \norm{\sum_{i=1}^n\theta_ig(u_i)}_2 \leq \sigma_g\sqrt{2nd\log(d/\delta)}
\end{equation}
where $g(u_i)$ is a zero mean sub-Gaussian random variable with variance $\sigma_g$.
\begin{proof} 

Since $\theta_i$ is chosen independently from each agent's type $u_i$, the variables $g(u_i)$ and $\theta_i$ are independent. Furthermore, we assume that the expected value $\E[g(u_i)]=0$.\footnote{Without this assumption, we run into identifiability issues: we cannot reconstruct the individual treatment effects $\left(\theta^*\right)^1,\dots,\left(\theta^*\right)^k$ without fixing some mean $\E[g(u)]$. For purposes of regret minimization, assuming $\E[g(u)]=0$ does not change our results.} Thus, we apply a high probability bound on the sum $\sum_{i=1}^n g(u_i)\theta_i$:
    \begin{align*}
        \norm{\sum_{i=1}^n g(u_i)\theta_i}_2
        &=\sqrt{\sum_{j=1}^k\left(\sum_{i=1}^n g(u_i)\theta^j_i\right)^2}\\
        &\leq \sqrt{\sum_{j=1}^k\left(\sum_{i=1}^n g(u_i)\right)^2} \tag{since, by assumption, $0\leq\theta^j_i\leq1$}\\
        &\leq \sqrt{\sum_{j=1}^k\left(\sigma_g\sqrt{2n\log(1/\delta_j)}\right)^2} \tag{by Chernoff Bound \lscomment{refer to theorem}}\\
        &\leq \sqrt{\sum_{j=1}^k\left(\sigma_g\sqrt{2n\log(k/\delta)}\right)^2} \tag{by Union Bound with $\delta_j=\delta/k$ for all $1\leq j\leq k$}\\
        &\leq \sigma_g\sqrt{2nk\log(k/\delta)}
    \end{align*}
\end{proof}
\end{lemma}

==> impossibility-changing-hidden-features.tex <==
\section{Impossibility of Recovering True Causal Effect under Changing Hidden Features}
\label{sec:impossibility}
% \lscomment{in progress...}
% Suppose that we adopt a model similar to that in \cref{sec:model}, where we deploy some $\theta$, the agent responds by choosing $x$, and we observe some true outcome based on the true parameter vector $\theta^*_x$. However, we may modify this model such that we introduce some hidden feature vector $h$, which is unobservable to the learner and changes when the agent modifies their features to report $x$. (Additionally, we get rid of the unobserved confounding variable $u$ without loss of generality.) 

% In this section, we will demonstrate that it is impossible to recover the true treatment effect $\theta^*_x$ for the observed features $x$ if we do not know the hidden features $h$ nor the treatment effect $\theta^*_h$ thereof. Consider that $y_i,x_i,h_i,\theta_i$ are indexed by round $i$. In general, we cannot recover the true parameter vector $\theta^*_x$ given access to a set of $T$ tuples $\{x_i,\theta_i,y_i\}_{i=1}^T$ without access to $h_i$. 


% \lscomment{I think we can't estimate $\theta^*_x$ if we have something like we don't observe that $h=0$ when $x=0$. This goes for the case where both $h$ and $x$ are observable, but $h$ is proportional to $x$; and for the case where $h$ is unobservable (so we don't know if $h=0$.}

% Consider a general linear model that demonstrates this effect, where at round $i$,
% \begin{align}
%     &(x_i,h_i) = M_i\theta_i\\
%     &y_i = \langle\theta^*_x,x_i\rangle + \langle\theta^*_h,h_i\rangle + \epsilon_i,
% \end{align}
% where $\theta_i\in\mathbb{R}^m$, $h_i\in\mathbb{R}^n$, $x_i\in\mathbb{R}^k$, and $M_i\in\mathbb{R}^{(n+k)\times m}$ is some conversion matrix (similar to our effort conversion matrix in \Cref{sec:model}). Assume that $\epsilon_i$ is a random zero mean subgaussian noise. Furthermore, assume that $x_i=h_i$ in every round $i$.

% In this simplified setting, we may attempt to estimate the conditional expectation 
% \begin{align*}
%     \E\left[y_i|x_i\right] 
%     &= \E\left[\langle\theta^*_x,x_i\rangle + \langle\theta^*_h,h_i\rangle + \epsilon_i|x_i\right]\\
%     &= \E\left[\langle\theta^*_x,x_i\rangle + \langle\theta^*_h,x_i\rangle + \epsilon_i|x_i\right]\\
%      &= \theta^*_x+\theta^*_h.\\
% \end{align*}

% In words, when we manipulate $\theta$ and observe some change in outcome $y$, we cannot decipher whether this effect is precipitated by $x$ or $h$. We only know that the expected outcome $y$ is given by $\theta^*_x+\theta^*_h$; without access to $\theta^*_h$, we cannot know $\theta^*_x$. \dncomment{change "without access" to something else. For example, if we knows the proportion between $\theta^*_x$ and $\theta^*_h$, then we can still recover the parameters}

% In numbers, let's say that we have a single sample $\{y_i=1,x_i=1,\theta_i=1\}$. In this case, 
% $1 = \theta^*_x + \theta^*_h + \epsilon_i$.
% \dncomment{simple setting: $y = \theta^*_x x + \theta^*_h h$, and there is only one action that increase both $x$ and $h$. If we deploy $\theta^*_x$ as our decision rule, and the agents take the action to increase both $x$ and $h$ by $1$. Then a learner who does not know about the hidden causal features will believe that the change in label (which is $2$) comes from change in $x$, implying the true model is $y = 2\theta^*_x x$. This can be generalized to settings where $x$ and $h$ are different or $h$ is not a function of $x$.}

% Generally speaking, it's possible to consider  to be any arbitrary error variable, zero mean or not. Without loss of generality, however, here let's assume it's zero mean.







    

% If both the observed and hidden features $x$ and $h$, respectively, are affected by the revealed $\theta$ and this effect is unknown, then we cannot recover the causal effect $\theta^*_x$ of the observed feature $x$ on $y$.

% In \Cref{fig:impossibility-dag}, we can see the causal diagram for this setting.

% \begin{figure}
%     \centering
%         \begin{tikzpicture}[node distance={15mm}, thick, main/.style = {draw, circle}] 
%         \node[main] (1) {$\theta$}; 
%         \node[main] (2) [right of=1] {$x$}; 
%         \node[main] (3) [below of=2] {$h$};
%         \node[main] (4) [right of=2] {$y$};
%         \draw[->] (1) -- (2); 
%         \draw[->] (1) -- (3);
%         %\draw[->] (2) -- (3);
%         %\draw (1) to [out=180,in=270,looseness=5] (1);
%         \draw[->] (3) -- node[below] {$\theta^*_h$} (4); 
%         \draw[->] (2) -- node[above] {$\theta^*_x$} (4); 
%         \end{tikzpicture} 
%     \caption{Causal graph of with changing hidden features}
%     \label{fig:impossibility-dag}
% \end{figure}

Assume we have the one-dimensional setting 

\begin{equation} \label{eq:x-and-h}
    y_t = \theta^*x_t + \beta^* h_t + g(u_t), 
\end{equation}


where $x_t$ are agent $t$'s observable, modifiable features, $h_t$ are the agent's unobsevable, modifiable features, and $g(u_t)$ is a function of agent $t$'s unobservable, unmodifiable features. We can assume $g(u_t) = 0$ in this section without loss of generality. If the relationship between $x_t$ and $h_t$ is unknown, then it is generally impossible to recover the true causal parameters $\theta^*$ and  $\beta^*$ since $h_t$ is never observed and any assessment rule $\theta$ deployed by the decision maker affects both $x_t$ and $h_t$, meaning that $\theta$ is not a valid instrument variable. This behavior can be seen in \Cref{fig:general-model-dag}. \khcomment{maybe say something about how this shows up in the Shavit paper}\\

On the other hand, if the relationship between $x$ and $h$ is known, there exist situations for which it is impossible to recover $\theta^*$ and $\beta^*$, even in the limit of infinite data. For example, if $x \in \mathbb{R}$ and $h = x$, the models $\theta^* = 1$, $\beta^* = 1$ and $\theta^* = 1.5$, $\beta^* = 0.5$ produce the same output for all $x \in \mathbb{R}$, making it impossible to distinguish between the two.

==> intro.tex <==
\section{Introduction}\label{sec:intro}

\dndelete{
\begin{figure}
    \begin{subfigure}[c]{0.48\textwidth}
         \centering
             \includegraphics[width=.8\textwidth]{figures/sciv-small-dag.png}
         \caption{model} 
         \label{fig:model-dag}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.48\textwidth}
         \centering
             \includegraphics[width=\textwidth]{figures/sciv-example-dag.png}
         \caption{example} 
         \label{fig:example-dag}
    \end{subfigure}
    \caption{Graphical model for our setting.\hhcomment{Where is effort in these diagrams?} Grey nodes are observed, white unobserved. Observable features $\vx_t$ (such as high school GPA in different subjects, SAT scores, etc.) depend on both the agent's private type $u_t$ (e.g., first-generation vs. non-first-generation students) \hhdelete{via initial features $\vz_t$ (e.g. the score student $t$ would receive on the SAT without studying)} and effort \hhdelete{conversion matrix $W_t$ (e.g. how much studying translates to an increase in SAT score for student $t$)} and assessment rule $\vtheta_t$ (via action $\va_t$, which could correspond to studying, taking an SAT prep course, etc.). An agent's outcome $y_t$ (e.g. their college GPA) is determined by their observable features $\vx_t$ (via causal relationship $\vtheta^*$) and type $u_t$ (via confounding term $g_t$, e.g. lack of resources, discrimination, etc). \hhcomment{We are still introducing new notation in a caption! We should simplify this caption to the extent possible. Do not add new parts to the example here.}}
    \label{fig:intro-dags}
\end{figure}
}

\begin{figure}
    \begin{subfigure}[c]{0.42\textwidth}
         \centering
             \includegraphics[width=\textwidth]{figures/sciv-model-full-dag.png}
         \caption{model} 
         \label{fig:model-dag}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.57\textwidth}
         \centering
             \includegraphics[width=1.1\textwidth]{figures/sciv-example-full-dag.png}
         \caption{example} 
         \label{fig:example-dag}
    \end{subfigure}
    \caption{Full graphical model for our setting with accompanying example. Grey nodes are observed, white unobserved. Observable features $\vx_t$ (e.g. high school GPA, SAT scores, etc.) depend on both the agent's private type $u_t$ (e.g., first-generation vs. non-first-generation students) via initial features $\vz_t$ (e.g. the SAT score or HS GPA student $t$ would get without studying) and effort conversion matrix $W_t$ (e.g. how much studying translates to an increase in SAT score for student $t$) and assessment rule $\vtheta_t$ via action $\va_t$, which could correspond to studying, taking an SAT prep course, etc). An agent's outcome $y_t$ (e.g. college GPA) is determined by their observable features $\vx_t$ (via causal relationship $\vtheta^*$) and type $u_t$ (via confounding term $g_t$, e.g. lack of resources, discrimination, etc).}
    \label{fig:intro-dags}
\end{figure}


Machine learning (ML) algorithms increasingly automate or inform consequential decision-making processes such as college admissions, credit scoring, and resume screening. In many of these settings, the deployed predictive models or assessment rules may prompt the assessed individuals to strategically adapt their behavior to receive more favorable predictions. Motivated by this type of behavior, a long line of work on ``strategic learning'' studies machine learning problems where models make predictions on strategic agents \citep{dong2018strategic,hardt2016strategic,  mendler2020stochastic, shavit2020strategic}. At a high level, much of the existing work in this literature has focused on developing robust algorithms that optimize predictive accuracy, while taking into account that agents will manipulate their features presented to the model.

Even though these algorithms for strategic learning can optimize predictive accuracy, they do not necessarily provide insights into the \emph{causal} relationships between the observable features and the outcomes, which are critical for many reasons. For example, knowledge of causal relationships can help agents identify meaningful interventions that can improve their outcomes, not just their assigned scores. Policymakers may use causal relationships to inform policy decisions and examine potential unfairness against certain sub-populations. \lsedit{For example, research showing the lack of causal effect that standardized test scores have on college performance has led many U.S. universities to abandon SAT and ACT scores in their admissions process \citep{allensworth2020gpasat,brooks2020cbsactsat}.} \swcomment{the refs are good, but the sentence seems a bit disconnected} Causal relationships can also help ensure robustness in predictive models so that they can reliably make accurate predictions even if the underlying covariate distributions have shifted over time.

In this work, we provide a general method for inferring causal relationships by establishing a novel connection between strategic learning and instrumental variable (IV) regression. By viewing the set of deployed predictive models as a form of instrumental variables, our framework can provably recover the causal relationships between the observable features and outcomes even in the presence of potential unobserved confounders. To describe our results, we will first introduce our model with college admissions as our running example. 

\xhdr{Our model.} Consider the setting in which a university decides whether to admit or reject applicants on a rolling basis (for example, \cite{psbwebsite}) based (in part) on how well they are predicted to perform {if admitted to the} university. We model such interactions as a game between a \emph{principal} (e.g. a university) and a population of \emph{agents} (e.g. applicants) {who arrive} sequentially over $T$ rounds. In each round $t$, the principal deploys a linear assessment rule $\vtheta_t$ that maps observable features $\vx_t$ (e.g. applicants' standardized test scores, math GPA, science GPA, humanities GPA, number of extracurricular activities, etc.) to a \emph{predicted outcome} $\hat{y}_t$ (e.g. an applicant's predicted college GPA). Then given this deployed rule, the agent at round $t$ arrives with their (unobserved) private type $u_t$. {For example, the type may indicate whether or not an applicant is a \emph{first-generation} college student.} Agent types are drawn independently from a fixed distribution. Each agent $t$ aims to optimize their predicted outcome by putting forth effort $\va_t$, which changes their observable features $\vx_t$ and subsequently their true outcome $y_t$. For instance, a student may choose to study individual subjects to improve their mastery of knowledge and relevant course grades, or they can take prep courses to improve their standardized test taking strategies and test scores. \khedit{\hhdelete{Even though one may ideally want to estimate the causal effect of each action or intervention available to each agent,} It is often unrealistic for the principal to directly observe efforts. Instead, the effort expended by an agent is reflected in their observable features. For example, a college application does not ask how much time an applicant has spent studying a certain subject, but it collects grades on relevant coursework. There is an underlying \emph{causal relationship} $\vtheta^*$ between observable features $\vx_t$ and outcome $y_t$, through these actions (reference figure here). In light of this, our goal is to recover the true causal relationship $\vtheta^*$ between observable features and outcome.} 
\hhcomment{If by 'action', you mean 'effort investment', use 'effort investment' consistently. }

\xhdr{Strategic regression as instruments.}
\iffalse
Under our model, we provide a general method to infer the causal relationship parameter $\vtheta^*$. The main challenge in estimating $\vtheta^*$ is that the features $\vx_t$ correlate with the ``noise'' term $g_t$, since they are both associated with the agent's private type $u_t$\lsedit{, e.g. the mean college GPA for first-generation students (with no college-educated family) may be lower than other students, due to institutional barriers}. As a result, standard techniques like ordinary least squares (OLS) will generally recover a biased estimate. To overcome this bias, we make the novel observation that the principal's assessment rule $\vtheta_t$ is a valid \emph{instrument}, since $\vtheta_t$ is independent of $g_t$ and $\vtheta_t$ influences the outcome $y_t$ only through its influences on an agent's action $\va_t$ and observable features $\vx_t$. By leveraging this observation, we can perform two-stage least squares (2SLS) to recover the causal relationship $\vtheta^*$. Our method applies to both \emph{off-policy} and \emph{on-policy} settings: one can directly apply 2SLS on historical data $\{(\vtheta_t, \vx_t, y_t) \}_{t=1}^T$, or the principal can intentionally deploy a sequence of varying assessment rules (by e.g., making small perturbations on a fixed rule $\vtheta_t$) and then apply 2SLS on the collected data.
\fi 
Under our model, we provide a general method to infer the causal relationship parameter $\vtheta^*$. {Since} the agent's private type $u_t$ may introduce a \emph{confounding effect} on the outcome, standard regression techniques like ordinary least squares (OLS) will generally recover a \emph{biased} estimate. To overcome this bias, we make the novel observation that the principal's assessment rule $\vtheta_t$ is a valid \emph{instrument}, and leverage this observation to perform two-stage least squares regression (2SLS) and recover the causal relationship $\vtheta^*$. Our method applies to both \emph{off-policy} and \emph{on-policy} settings: one can directly apply 2SLS on historical data $\{(\vtheta_t, \vx_t, y_t) \}_{t=1}^T$, or the principal can intentionally deploy a sequence of varying assessment rules (by e.g., making small perturbations on a fixed rule $\vtheta_t$) and then apply 2SLS on the collected data. \khcomment{What do you guys think now? I cut out a fair bit of the technical details to make it easier to understand for the reader. I'm hoping that keeping things general, along with our "simple" figures will be enough for the reader to get a high-level idea of what we're doing.}

\xhdr{Two relevant optimization problems.} We then study two natural optimization objectives, for which we can build our solutions given our knowledge of the causal relationship $\vtheta^*$. We first study \emph{agent outcome maximization}: how to use assessment rules $\vtheta_t$ as a form of intervention that incentivizes the population of agents to invest their efforts optimally so that their average outcomes ($y$) are maximized. Using parameters estimated during our 2SLS procedure, we can solve an optimization problem to recover an estimate of the assessment rule which maximizes expected agent outcome.
\iffalse
We show that our 2SLS method nicely recovers \khedit{an estimate of $\E[W_t W_t^\intercal] \vtheta^*$ in its second stage} \khdelete{the two relevant estimates $\E[W_t W_t^\intercal]$ and $\vtheta^*$ in its stages}, which allows us to maximize the expected agent outcome objective, which can be re-written as $\langle \vtheta_t, \E[W_t W_t^\intercal] \vtheta^* \rangle$. 
\fi
We then study the problem of \emph{predictive risk minimization} that aims to minimize $\E[(\hat y_t - y_t)^2]$\khedit{, the expected squared difference between an agent's \emph{true} outcome and the outcome predicted by the principal}. Compared to standard regression, this is a more challenging objective since both the prediction $y_t$ and outcome $\hat y_t$ depend on the deployed rule $\vtheta_t$, which leads to a non-convex risk function. We show that the knowledge of $\vtheta^*$ enables us to compute an unbiased estimate of the gradient of the predictive risk. As a result, we can apply stochastic gradient descent to find a local minimum of the predictive risk function. \khcomment{Would like to say that performative prediction does not work well in practice in our setting.}

\iffalse
\khcomment{
Storyline:
\begin{itemize}
    \item A growing line of work advocates for studying people's responses to algorithmic decision making tools---e.g., ways in which decision subjects can change their attributes to receive more desirable decisions.
    \item The reasons that are often cited to support this call are: (1) investigating the ethicality (e.g., fairness) of a decision rule often requires knowledge of the \emph{true} relationships among certain variables of interest. (2) A good decision rule is one that contributes to better societal outcomes in the \emph{long-run}---by encouraging people to take steps that improve their future welfare. 
    \item Viewed in this light, algorithmic decision rules can serve as a means for social scientists and policy makers alike to understand and improve social outcomes.
    \item Social scientists can treat these tools as a form of intervention that allows them to causally reason about the underlying dynamics (recovering true relationship between observable features and outcomes). Policy makers can design dynamic decision rules that nudge the population in their planned direction (maximizing social welfare in the long-run).
\end{itemize}}

\subsection{Running Example}
\khcomment{This section is for our benefit only}
Consider a university that admits students on a rolling basis and decides which applicants to admit based (in part) on how well they expect them to perform in university. The university uses an assessment based on standardized test scores, high school GPA (consisting of \emph{math}, \emph{science}, and \emph{humanities} GPA), number of extra-curricular activities, etc. for their admissions policy. There are two types of applicants: 1) \textit{first-generation students} who are the first of their family to go to college and 2) non-first generation students. These two types may have different distributions on their initial features, e.g. first-generation students may start off with lower standardized test scores or high school GPA, on average. The two different groups may also expend different amounts of effort to improve their features, e.g. a higher proportion of non-first generation students may have access to private tutoring, making it easier for them to improve their standardized test scores or GPA than first-generation students who need to study on their own. Finally, the true baseline outcome (success at university, measured by college GPA) of the two groups may differ beyond the causal effects of their observable features as well. These differing baseline outcomes can be modeled by a confounding term $g_t$ for each of the two types. In our college admissions example, the baseline university GPA for first-generation students may be lower due to institutional barriers --e.g. discrimination, lack of resources, etc.-- may not be present for non-first generation students.


Consider the setting in which a university decides whether to admit or reject applicants on a rolling basis (for example, \cite{psbwebsite}) based (in part) on how well they are predicted to perform in university. We study a game between a \emph{principal} (e.g. a university) and a population of \emph{agents} (e.g. applicants) over $T$ rounds. In each round $t$, the principal chooses to deploy an assessment rule $\vtheta_t \in \mathbb{R}^m$ that \textit{linearly} maps an agent's observable features to a \emph{predicted outcome} $\hat{y}_t \in \mathbb{R}$ (e.g. an applicant's predicted college GPA). At time $t$, a new agent indexed by $t$ arrives with their \emph{observable} features $\vx_t \in \mathbb{R}^m$ (e.g. applicants' standardized test scores, math GPA, science GPA, humanities GPA, number of extracurriculars, etc.). The principal assesses the applicant by computing
\begin{equation}\label{eq:predicted-outcome}
    \hat{y}_t = \mathbf{x}_t^\top \vtheta_t.
\end{equation}
The linearity assumption on the relationship between observable features $\vx_t$ and the predicted outcome $y_t$ has been adopted in practice, e.g. in college GPA prediction based on high school GPA and SAT scores \citep{zwich} and is reflected in prior models of strategic learning~\citep{shavit2020strategic, dong2018strategic, BechavodLWZ21}.

\xhdr{Agent features and causal actions.}
If an applicant knows what features they will be evaluated on, they can do things to improve their chances of being admitted, like studying physics to improve their science GPA, taking an SAT prep course, or joining more extracurriculars. While some actions may be \emph{causally} related to college success, others may not be. For example, studying physics could be considered causally related to success in college, since this improves a student's knowledge and background on subjects they may learn more about at university. Even a student chooses not to study science in college, developing good problem solving techniques may be useful for other domains such as economics or computer programming. On the other hand, taking an SAT prep course may \emph{not} be causally related to success in college, especially if the prep course teaches students test-specific strategies that don't generalize well to other learning settings. Let agent $t$'s \emph{causal} relationship between actions and outcomes be defined by the vector $\boldsymbol{\mu}_t^*$. In our example, $\mu_{t,SAT}^*$ would be near zero for each student $t$.

While the principal may want to incentivize agents to invest effort in actions which are causally related to positive outcomes (e.g. those with high $\mu^*$ values), it is usually hard to learn which actions are causal in practice since agent actions are rarely observed. Instead, the principal usually only has access to the agent's observable features. With this in mind, a natural goal for the principal is to \emph{learn} the true underlying relationship between observable features and positive outcomes, and \emph{incentivize} agents to invest effort to improve these features by placing high emphasis on them in the assessment rule they choose to deploy. For example, if a university knew that studying for science coursework was causally related to success in college and studying for the SAT was not, they would want to increase the weight they place on science GPA and decrease the weight they place on students' SAT scores when making admissions decisions.
\fi 

%\swdelete{\subsection{Summary of Results}
%Our contributions are as follows. We cast the strategic classification problem as two-stage least-squares regression, a form of IV regression. Because of this, we are able to recover an estimate of the true relationship between observable features $\vx_t$ and outcome $y_t$ from $\{(\vtheta_t, \vx_t, y_t)\}_{t=1}^T$ data in the presence of confounding terms without any prior knowledge about the agent population. Moreover, if the decision rules $\{\vtheta_t\}_{t=1}^T$ are sufficiently random and the agent population is sufficiently well-behaved, the distance $\| \vtheta^* - \widehat{\vtheta} \|_2$ between the causal parameters and the estimate obtained via 2SLS shrinks at a rate $\mathcal{O}(\frac{1}{\sqrt{T}})$. Recovering the true underlying relationshp between observable features and outcome may not be the only goal of the principal in strategic classification settings. Another competing objective, agent outcome maximization, aims to deploy the decision rule $\vtheta^{AO}$ which maximizes the expected outcome of an agent drawn from the population. Using parameters from our 2SLS estimate of $\vtheta^*$, we are able to recover an estimate of $\vtheta^{AO}$ by solving a linear program. Under the same nicety conditions on the deployed decision rules and agent population, the distance between $\vtheta^{AO}$ and our estimate also shrinks at rate $\mathcal{O}(\frac{1}{\sqrt{T}})$. Finally, we explore the use of natural learning dynamics when minimizing predictive risk. We show that while the methods of \cite{mendler2020stochastic} may not converge to performatively stable points in our setting, running online gradient descent does. We also identify several special cases of our setting in which running online gradient descent converges to performatively optimal points.}

==> model.tex <==
\section{Model}\label{sec:model}

%\hhcomment{Figure 2 is very helpful and clarifies many things. The only issue I see with the example is the direct link between $u$ and $y$. College GPA is often a deterministic function of grades (x), and there is no direct link between institutional barriers and GPA given grades. One solution would be to change college GPA to 'college graduation'. } \khcomment{Why don't we just talk about things more generally? An agent's 'type' encapsulates everything about them (such as intelligence, charisma, etc.), which does have a direct link with college GPA.}

In our model, the principal deploys a linear assessment rule $\vtheta_t \in \mathbb{R}^m$ at each time-step, and assigns agent $t$ a predicted outcome $\widehat{y}_t = \vx_t^\top \vtheta_t \in \mathbb{R}$, where $\vx_t \in \mathbb{R}^m$ are the agent's observable features. 
We assume that the agent best-responds to the assessment rule $\vtheta_t$ by strategically playing a set of observable features $\mathbf{x}_t$ in order to receive a favorable predicted outcome $\hat{y}_t$, subject to some \emph{effort} cost $c(\cdot)$ associated with modifying their feature values. For example, a prospective student might take more standardized test preparation, which could significantly improve their SAT scores, as well as have a slight positive impact on their math and humanities GPA. Specifically, we assume agent $t$'s observable features take the form 
\begin{equation*}
    \mathbf{x}_t = \mathbf{z}_t + W_t \mathbf{a}_t,
\end{equation*}
where $\vz_t \in \mathbb{R}^m$ are agent $t$'s initial, \emph{unobserved} feature values, $W_t$ is agent $t$'s \emph{effort conversion matrix}, and $\mathbf{a}_t \in \mathbb{R}^d$ is the \emph{action} agent $t$ takes in response to the assessment rule $\vtheta_t$. The effort conversion matrix $W_t$ maps changes in effort to changes in observable features. The $(k,j)$-th entry of $W$ defines the change in the $k$-th observable feature $x_{t,k}$ for a one unit increase in the $j$th coordinate of the effort vector $\mathbf{a}_t$. \swdelete{For example, studying for a standardized test might correspond to a column $W_1 = (10, 0.4, 0, 0.3)^\intercal$ in the effort conversion matrix, in which the four entries represent a large increase in SAT score, small increase in math GPA, no change in science GPA, and a small increase in humanities GPA, respectively.} Importantly, our model allows for the effort conversion matrix $W_t$ to vary between different types.\swcomment{we didn't define types}

We assume that the agent selects their effort profile $\mathbf{a}_t$ in order to maximize their predicted outcome $\hat{y}_t$, subject to a quadratic cost penalty, a common assumption in the strategic classification literature (\cite{shavit2020strategic, mendler2020stochastic, dong2018strategic}). In this work, we choose the quadratic cost $c(\va_t) = \frac{1}{2} \|\va_t\|^2_2$. Specifically, we assume that agents select their action $\va_t$ by solving the following optimization problem:
\begin{equation*}
    \mathbf{a}_t = \argmax_{\va} \left\{ \hat{y}_t -  \frac{1}{2} \|\mathbf{a}\|^2_2 \right\}
\end{equation*}
We can obtain a closed-form solution for agent $t$'s action $\va_t$ by substituting in the expression for agent $t$'s predicted outcome $\hat{y}_t$ and observable features $\vx_t$. Doing this, we see that $\va_t$ takes the form 
\begin{equation*}
    \mathbf{a}_t = W_t^\top \vtheta_t.
\end{equation*}

\iffalse
It is now possible to formally define the causal relationship $\boldsymbol{\mu}^*_t$ between actions and outcomes for an agent $t$ as 
\begin{equation*}
    \boldsymbol{\mu}^*_t = W_t^\top \vtheta^*.
\end{equation*}
$\boldsymbol{\mu}^*_t$ represents how much actions are causally related to outcomes for agent $t$. Note that $\boldsymbol{\mu}^*_t$ may vary from agent to agent. For example, some students may have an easier time mastering the subjects necessary for success in college than others, meaning that they need to expend less effort in order to achieve the same collegiate success.

In order for a unique $\vtheta^*$ to exist, the following condition on observable features $\vx_t$ and actions $\va_t$ must hold.
\begin{assumption}[Identifiability]
    For every agent $t$, no two different actions should be able to produce the same set of observable features. In other words, if $\va_t \neq \va_t'$ then $\vx_t \neq \vx_t'$.
\end{assumption}
\hhcomment{Doesn't this assumption imply that one can uniquely infer actions from observables? If so, this casts doubt on our premise that the principal cannot observe the actions directly.} \khcomment{I don't think so, since the principal never gets to observe $W_t$.}
If this assumption does not hold, there could be multiple $\vtheta^*$ which map to the same $\boldsymbol{\mu}_t^*$. However, as long as the principal has access to sufficiently many observable features when predicting agent outcome this assumption should hold.
\hhcomment{So the above assumption is stronger than invertibility of $W$, right? If so, we should clearly say why we need this extra strong assumption.}
\fi 

\iffalse
The agent's private type $u_t$ includes their unmodified feature $\vz_t \in \mathbb{R}^m$ before any effort $\va_t$, their effort conversion matrix $W_t \in \mathbb{R}^{m \times d}$, which determines how their efforts translate to changes in $\vx_t$, and their baseline outcome $g_t$, that captures other unobserved factors that influence the outcome. 
\fi 

\xhdr{True outcome model.} \emph{After} each round, the principal gets to observe the agent's true outcome $y_t \in \mathbb{R}$ (e.g. an applicant's true college GPA), which takes the form
\begin{equation*}
    y_t = \mathbf{x}_t^\top \vtheta^{*} + g_t
\end{equation*}
Here $\vtheta^*$ is the \emph{true} relationship between an agent's observable features and outcome, and $g_t \in \mathbb{R}$ is an unobserved confounding term which captures the dependence of agent $t$'s outcome $y_t$ on factors other than their observable features.
An example of a confounding term in our college admissions example may be institutional barriers --e.g. discrimination or lack of resources, which could cause first-generation students to have less collegiate success than non-first generation students students, irregardless of their observable features. In this setting, $g_t$ would be negative for first-generation students and positive for non-first generation students, on average. 
\hhcomment{The example above should have appeared way earlier.}
\dndelete{
\begin{figure}
    \begin{subfigure}[c]{0.42\textwidth}
         \centering
             \includegraphics[width=\textwidth]{figures/sciv-model-full-dag.png}
         \caption{model} 
         \label{fig:model-dag}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.57\textwidth}
         \centering
             \includegraphics[width=1.1\textwidth]{figures/sciv-example-full-dag.png}
         \caption{example} 
         \label{fig:example-dag}
    \end{subfigure}
    \caption{Full graphical model for our setting with accompanying example. Grey nodes are observed, white unobserved. Observable features $\vx_t$ (e.g. high school GPA, SAT scores, etc.) depend on both the agent's private type $u_t$ (e.g., first-generation vs. non-first-generation students) via initial features $\vz_t$ (e.g. the SAT score or HS GPA student $t$ would get without studying) and effort conversion matrix $W_t$ (e.g. how much studying translates to an increase in SAT score for student $t$) and assessment rule $\vtheta_t$ via action $\va_t$, which could correspond to studying, taking an SAT prep course, etc). An agent's outcome $y_t$ (e.g. college GPA) is determined by their observable features $\vx_t$ (via causal relationship $\vtheta^*$) and type $u_t$ (via confounding term $g_t$, e.g. lack of resources, discrimination, etc).}
    \label{fig:intro-dags}
\end{figure}
}
\lsdelete{
\begin{figure}[]
 \centering
     \begin{tikzpicture}[node distance={15mm}, thick, main/.style = {draw, circle}] 
     \node[draw,circle,fill=lightgray] (1) {$\vtheta_t$}; 
     \node[draw,circle,fill=lightgray] (2) [right of=1] {$\vx_t$}; 
     \node[main] (3) [below of=2] {$u_t$};
     \node[draw,circle,fill=lightgray] (4) [right of=2] {$y_t$};
     \draw[->] (1) -- node[above] {$\va_t$} (2);
     \draw[->] (3) -- node[left] {$\vz_t$, $W_t$} (2);
     % \draw (1) to [out=180,in=270,looseness=5] (1);
     \draw[->] (3) -- node[below right=-0.15cm] {$g_t$} (4);
     \draw[->] (2) -- node[above] {$\vtheta^*$} (4);
     \end{tikzpicture} 
 \caption{Graphical model for our setting. Grey nodes are observed, white unobserved. Observable features $\vx_t$ (such as high school GPA in different subjects, SAT scores, etc.) depend on both the agent's private type $u_t$ (e.g., first-generation vs. non-first-generation students) via initial features $\vz_t$ (e.g. the score student $t$ would receive on the SAT without studying) and effort conversion matrix $W_t$ (e.g. how much studying translates to an increase in SAT score for student $t$) and assessment rule $\vtheta_t$ (via action $\va_t$, which could correspond to studying, taking an SAT prep course, etc.). An agent's outcome $y_t$ (e.g. their college GPA) is determined by their observable features $\vx_t$ (via causal relationship $\vtheta^*$) and type $u_t$ (via confounding term $g_t$, e.g. lack of resources, discrimination, etc.).} 
 \label{fig:model-dag}
\end{figure}
}% end lsdelete


\iffalse
When thinking about $g_t$, it helps to consider two types of applicants ---\textit{first-generation} students (the first in their family to go to college) and non-first-generation students (who are not): first-generation students may have lower baseline college GPA than legacy students due to institutional barriers or lack of resources. Together these factors determine the observable features and outcomes via two equations (also see Figure~\ref{fig:model-dag}):
\begin{equation*}
    \vx_t = \vz_t + W_t \va_t, \qquad y_t = \langle \vtheta^*,  \vx_t \rangle + g_t,
\end{equation*}
where $\vtheta^* \in \mathbb{R}^m$ is the \emph{causal relationship parameters} between the observable features and outcome we wish to recover. For example, first-generation students and non-first-generation students may have substantially different effort-conversion matrices $W_t$, since a smaller proportion of first-generation students may have access to resources such as private tutoring which could help them improve their test scores and course grades more efficiently.
\fi 




The agent's private type $u_t$, drawn from some arbitrary distribution $\mathcal{P}$, specifies the agent's $(\vz_t, W_t, g_t)$ tuple. Note that we make no assumptions on the distribution over $\mathcal{P}$, meaning $\vz_t$, $W_t$, and $g_t$ may be correlated with one another. Because of this, ordinary least squares will generally \emph{not} be a consistent estimator for $\vtheta^*$ (see \Cref{sec:ols} for more details). Instead, if we wish to estimate the true relationship between observable features and outcomes, a method which decouples the contributions of the agent's observable features $\vx_t$ and confounder $g_t$ to his outcome, such as instrumental variable regression, must be used. Estimating this true relationship is important because features which are primarily modifiable through causal actions will have a strong relationship with positive agent outcomes, whereas features which are easily modifiable through non-causal actions will not. 




\iffalse
\khcomment{old summary of Shavit}
They provide algorithms for optimizing three decision-maker objectives: agent outcome maximization, prediction risk minimization, and parameter estimation. Our setting differs from theirs in a number of important aspects. First, \cite{shavit2020strategic} assume an agent's hidden features can be changed through strategic manipulation, while we assume that an agent's private type (which includes the agent's unobservable features) is an unmodifiable property of the agent. Ours is ostensibly a less general setting than \cite{shavit2020strategic}: however, we demonstrate that parameter recovery is, in general, impossible if agents' hidden features can be manipulated. This is likely why \cite{shavit2020strategic} assume that all features of an agent are observable to do causal inference. This illuminates a second difference, that we can recover causal parameters without observing all agent features (their private type captures unobservable features). Third, whereas \cite{shavit2020strategic} optimize for a single objective at a time, we identify natural learning dynamics which either minimize prediction risk or maximize agent outcome while estimating causal parameters. Moreover, we provide a regret-based analysis: \cite{shavit2020strategic} do not.

Finally, \cite{shavit2020strategic} assume a homogeneous population wherein agents’ initial features are identically distributed. However, this may not be a realistic assumption in many cases: \cite{hu2020disparate} explicitly consider strategic learning in a ``world of social stratification'' wherein an advantaged group of people has (on average) better initial features and exerts less effort to change their features than a disadvantaged group (p.2). Our work extends this heterogeneous setting so that an agent's \emph{unobserved type} determines how their initial features are distributed, influences the reward that the agent receives and how much effort is needed to change their features (see \Cref{fig:model-dag} for our model). \dncomment{Currently using same effort conversion matrix for everyone, but if we can have different matrices, then add to this sentence?} Consider an example to justify this setting: first-generation students, on average, have worse educational records when applying to university than continuing-generation students; also, first-generation students generally perform worse than continuing-generation students in university ---possibly due to discrimination or other institutional barriers. Due to the confounding between agents' unobserved initial features and the true outcomes they receive, ordinary least squares regression ---such as in \cite{shavit2020strategic}--- will produce a biased estimator of agents' causal parameters in this case. We remedy this problem by considering the assessment rule an instrumental variable (IV) and consistently recovering causal parameters via IV regression.
\fi 



==> old-materials.tex <==
\section{Introduction}


\swcomment{

\begin{itemize}
    \item Related work.
    \item describe how this model can still be viewed as an MAB problem if we have fully BIC---that is, we average out the baseline reward across types
\end{itemize}


}




In many online recommendation systems, including Netflix, Amazon, Yelp, Stubhub, and Waze, users are both consumers and producers of information. Users make their selections based on recommendations from the system, and the system collects data about the users' experiences to provide better-quality recommendations for future users. To ensure the quality of its recommendations, the system typically needs to balance between \emph{exploration}---selecting potentially suboptimal options for the sake of acquiring new information---and \emph{exploitation}---selecting the best option given the available information. However, there is an inherent tension between exploration and the users' incentives---since each user is primarily concerned with their short-term utility, their incentives naturally favor exploitation. 

To resolve this tension between exploration and incentives, a long line of work started by~\cite{KremerMP13, mansour2015bic} has studied mechanisms that incentivize users to explore by leveraging the information asymmetry between the recommendation system and users \citep{MansourSSW16, ImmorlicaMSW19, SS20}. These papers consider a simple multi-armed bandit model, where the recommendation system is a social planner who interacts with a sequence of self-interested agents. The agents arrive one by one to choose from a given set of alternatives (or called actions or arms) and receive a reward for their choice. Upon the arrival of each agent, the social planner provides a recommendation (one of the alternatives) that influences the agent's selection. The problem is to design a recommendation policy that incentivizes the agents to perform exploration and in the long run maximize the cumulative rewards of all the agents.  

Prior work on "incentivizing exploration" typically approaches the problem by enforcing \emph{Bayesian incentive-compatibility} (BIC) for every agent---that is, it is in each agent's interest to follow the planner's recommendation even if such action is inferior according to their prior belief. To achieve BIC, these mechanisms typically need to assume a strong assumption that all of the agents and the planner share a \emph{common prior} over the rewards of actions. However, in reality, agents tend to be inherently heterogeneous in terms of their beliefs and perceived rewards. In particular, some agents can have a stronger bias that favors one action over others and different agents. Moreover, even if the actions have the same effects on all of the agents, their realized or observed utilities can be different. For example, different patients taking the same drug may report levels of pain and different drivers taking the same route may have different commute time. 

\begin{example}[Motivating Example: Sales Campaign] A bank wants to estimate the return on investment (ROI) of a sales intervention wherein a salesperson offers a high rate of return on a savings account if a client deposits a large sum of money into the account.

On each day $t$, a client is assigned a particular sales person, who may or may not take the intervention. If the salesperson offers the intervention ($x_t=1$ in our model) the bank incurs a cost $c_t$ to pay out on the savings account (which is given by the rate of return and the deposit amount) and generates revenue $r_t$, since the clients may be more likely to open up other accounts, e.g. credit cards or investment accounts, which generate profit over time. If the salesperson takes the control  ($x_t=0$ in our model), the cost and revenue are zero. In our model, the population return caused by the intervention is given by $\theta = \E[r_t-c_t | x_t=1]$ and the instances of $r_t-c_t$ are randomly given by $\theta x_t + \epsilon_t$.

As such, the bank could estimate the return $\theta$ caused by the intervention by simply calculating the mean return under the intervention or the control. However, the clients also generate some baseline revenue, which is independent from the sales intervention. This baseline revenue $g(u_t)$ is given by the client’s \textit{type} ($u_t$ in our model), which also determines the salesperson’s expectation of the cost and revenue of the sales intervention. For example, the client’s type could be that they're a wealthy law firm with a lot of investable assets: the client generates high baseline revenue because they have a lot of money invested in the bank, of which the bank takes a percentage fee; as well, the salesperson anticipates that the law firm will deposit a lot of money into the savings account --incurring high cost $c_t$-- without opening any additional accounts --low revenue $r_t$.

Notably, the bank only observes whether or not the salesperson takes the intervention and the net revenue $y_t$ (given in equation~\eqref{eq:reward-model}). Since the unobserved baseline revenue $g(u_t)$ is correlated with the salesperson’s choice $x_t$, this causes confounding and the bank can no longer estimate the intervention return by simply taking the mean.

As such, the bank deploys a daily recommendation platform for the sales team, so as to optimize the bank's overall net revenue. Each day, the recommendation $z_t$ is based on the history $H_t$ of the intervention, i.e. all the past recommendations $z_t$, actions taken $x_t$, and the net revenues $y_t$.

Each salesperson $t$, considers this recommendation and their prior belief about the expected net revenue caused by the sales intervention, to decide whether to take the intervention or not, as in equation~\eqref{eq:two-arm-general-selection-function}. \lscomment{The recommendation may sway some risk-averse salespeople to take the intervention and some risky salespeople to take the control, causing more variability over the types.} The bank uses the recommendation $z_t$ as an instrument to better estimate the net revenue caused by the intervention $\theta$, as we expand upon in the following section.

\lscomment{End of bank example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse

Consider a corporation that  wants to estimate the average effect of interventions that the sales team can take on their customers (e.g. outreach phone calls, offering discounts or free credits), on the revenue of their customers. The corporation wants to deploy a daily recommendation platform for the sales team, so as to optimize operations and learn best practices. We consider a simplified setting where there is only a single type of intervention and the corporation does not know its return on investment (ROI). On each day $t$, a customer is assigned a particular sales person, who may or may not take the intervention. We assume that the effect of the intervention is observed at the end of the day (e.g. whether a purchase was made; this can also be replaced by some other short-term proxy/signal of long-term revenue, if long-term revenue is the goal).\footnote{The setting can also be easily relaxed with batches of customers each day (this can be thought as a method of online experimentation and active learning from the corporation).} The corporation is trying to identify the net effect of the intervention: this corresponds to some revenue lift $\delta$ minus a (potentially known) intervention cost $c$.

We model this scenario as bandits learning of two actions, where action 1 is "not taking intervention" and action 2 is "taking intervention". Then the net effect of the intervention is $\theta^2 = \delta - c$. Moreover, when no intervention is taken, then no lift in the revenue is observed and no cost is paid, rather the customer is expected to generate an organic, baseline amount of revenue $g(u_t)$, and so $\theta^1 = 0$. Here $u_t$ is an unobserved type of the customer, that is not known to the principal, but is observed by the sales person. This signal $u_t$ essentially captures the information asymmetry of the setting: sales people know more about the customers that they are working with than the corporation (e.g. whether they are about to grow, whether they are about to sign a big contract, whether they are about to make a big purchase because of increase in demand on the customer side). So at the end of the day, the customer generates revenue:
$y_t = \theta^{a} + g(u_t) + \epsilon_t$,
where $a\in \{1, 2\}$. The information asymmetry (i.e. that the agents know $u_t$ but the principal doesn't) is exactly what causes the endogeneity problem in the choice of the agents and why an instrumental variable approach is necessary. The goal of the principal is to maximize revenue, or more concretely minimize expected regret in terms of revenue, i.e.:
\begin{equation}
    R(T) = T\theta^{a^*} - \sum_{t} \theta_t^{X_t} 
\end{equation}
where $a^*=1$ if $\delta<c$ and $a^*=2$ if $\delta\geq c$.

The principal does not know the ROI $\theta^2$, and as is typical in corporate settings, will compensate the salesperson as a fraction of the observed revenue $y_t$, whenever an intervention is made.\footnote{Potentially this compensation structure could change once the ROI is estimated by the principal, which would then remove the endogeneity problem, but until the ROI is pin-pointed, this is a typical compensation schemes in corporate settings.} Thus, the salesperson receives reward:
\begin{equation}
    r_t = \beta\, y_t
\end{equation}
for some $\beta\in (0, 1]$. We also assume that each sales person has some outside option of collecting a reward $\pi$ (e.g. by doing what they would normally be doing and not following the principals recommendation). Thus the salesperson will take the action $a=1$ only if they expect a positive net benefit:
\begin{equation}
    X_t = 1 + \1\left\{\E_{\theta\sim \cP}[\theta^2] + g(u_t) \geq \pi/\beta\right\} = 1 + \1\left\{\E_{\delta\sim \cP}[\delta] - c + g(u_t) \geq \pi/\beta \right\} 
\end{equation}

In the case of two types $u_t\in \{1, 2\}$, We will also assume for simplicity that a priori both types will prefer to take the intervention. However, we assume that there is a probability under their prior beliefs that $\theta^2+g(u_t) \leq \pi/\beta$ for both types. At the end of the day the principal and the salesperson observe $y_t=\theta^a + g(u_t) + \epsilon_t$. This example is a special case of our framework, where $\theta^2=\delta - c$ and all agents have a uniform prior $\cP$ on $\delta$, with $c$ known. Moreover, $\phi(u_t)=\pi/\beta + c - g(u_t)$, for a known $\pi$, but a type $u_t$ unobserved by the principal and only observed by the agent.\fi

\end{example}


To explicitly capture the underlying heterogeneity across agents, we study a new model in which each agent has unobserved private type that determines both their prior preferences across the actions and their action-independent confounding shift in the rewards. Since the heterogeneity of the agents confounds the observed rewards, we draw techniques from instrumental variable regression to estimate the reward effects across the actions.
In particular, we take a novel view that  the planner’s recommendations can serve as a form of instrumental variables (IV) that only affect agents’ arm selection but not the observed rewards. We construct such IVs by carefully mapping the history–the interactions between the planner and the previous agents to a random recommendation. By running IV regression, our mechanism obtains a reliable estimate of reward effect of each action and in turn incentivize the agents' selections to converge on the optimal action.

A major advantage of our IV-based mechanism is that we no longer need to enforce BIC for all agents. Our algorithm can estimate the action effects accurately, as long as the recommendations induce variability in the agents' selections. An important special case is when a fraction of the types are more willing to explore an action that a-priori inferior. Furthermore, as soon as the mechanism obtains a sufficiently accurate estimate on the action effects, the policy can then be BIC for the remaining types. We demonstrate such partially BIC policy can significantly improve the regret bounds of a fully BIC policy obtained by extending the algorithm of \cite{mansour2015bic} to our setting. Moreover, our IV-based mechanism also mitigates the negative externality that their fully BIC policy imposes on a subgroup of agents. The reason is that their fully BIC policy will necessarily impose a longer exploration phase on agents of all types, which incurs unnecessary additional regret on agents who are more willing to follow the planner's recommendations. Since our IV-based mechanism does not require fully BIC to obtain accurate estimates, it also mitigates such unfair externality.

\paragraph{Additional motivating examples}
The trade-off between exploration and exploitation in the bandit setting could be observed in various scenarios that highlights the need for a natural instrument to help estimate the reward of each arm.\\
One such scenario concerns the lending discriminatory of a bank to different businesses, big and small. A bank is trying a sales campaign where a loan officer can offers a business client a low interest loan as an intervention. If they offer the loan, the bank incurs cost based on how much money the business takes out and if they default. Businesses generate baseline revenue that depends on its type and is independent of the intervention, i.e. big businesses already have more investment with the bank. so they generate more revenue regardless of the loan offer. Whether the loan officer offers the loan depends on the business type: they are biased against small businesses since they are more likely to default. The intervention choice is correlated with the baseline revenue and causes confounding effect. This calls for an instrument, which in this case is the bank's recommendation, to accurately estimate the effectiveness of the loan. By giving recommendation to induces variability, the bank can incentivizes loan officers to lend to small businesses. Thus, we can also prevent the discrimination against one type of business in this setting. 

\subsection{Related Work}




\textbf{Organization.} In this workshop version, we will present our formal model (Sec.\ref{sec:model}) and illustrate key ideas of our mechanism in a simple setting of two private types and two arms (Sec. \ref{sec:two-arms-two-priors}). We defer the fully general results and details to the full version.

\section{Model}\label{sec:old-model}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Previous model %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{} We study a sequential game between a \textit{learner} and a sequence of strategic \textit{agents} over $T$ rounds, where $T$ is known to the learner. In each round $t$, an entirely new agent indexed by $t$ arrives with their \emph{private type} $u_t$ drawn independently from a distribution $\cU$ defined over the set $U$ of all privates types, as well as their \emph{private true features} $x_t\in\mathbb{R}^n$, where $n$ is the total number of features.

Each agent $t$ receives a signal which contains the \emph{revealed treatment effect} $\tilde{\theta}\in\mathbb{R}^n$ from the learner, the agent strategically selects a set of features $\tilde{x}_t(\tilde{\theta})\in\mathbb{R}^n$ --which is a function of the learner's revealed $\tilde{\theta}$-- to disclose to the learner, and receives a reward $y_t\in\mathbb{R}$.

\paragraph{Reward} Given the agent's choice of feature vector $\tilde{x}_t\in\mathbb{R}^n$, the observed outcome $y_t$ for each agent $t$ is given by 
\begin{equation}
    \label{eq:reward-model}
    y_t = \langle \theta, \tilde{x}_t \rangle + g(u_t) + \epsilon_t,
\end{equation}
where $\theta\in\mathbb{R}^n$ denotes the unknown exogenous \emph{treatment effect}, the term $g(u_t)$ denotes an unobservable \emph{confounding variable} that depends on the agent's private type $u_t$, and the term $\epsilon_t$ denotes an independent reward noise vector with a subgaussian norm of $\sigma_{\epsilon}$ and conditional expectation $\E[\epsilon_t \mid x_t, u_t] = 0$. 

Both $g(u_t)$ and $\epsilon_t$ are unobserved by the learner. The learner's objective is to maximize the expected observed reward of all agents over all $T$ rounds, i.e. the learner's objective is to find a set $\tilde{\theta}^*$ of revealed $\tilde{\theta}_t$ over all rounds $t$ such that 
\begin{equation}
    \label{eq:learner-objective}
    \tilde{\theta}^* \in \argmax_{\tilde{\theta}}\, \E\left[ \langle \theta, \tilde{x}_t(\tilde{\theta}_t)\rangle \right]
\end{equation}


The utility for an agent $t$ is different than the observed reward insofar as the agent incurs some cost for revealing a set of features $\tilde{x}_t$ that deviates from their true features $x_t$. Let the utility for agent $t$ be:
\begin{align}
    \label{eq:reward-model-agent}
    y_t^{\text{agent}} :=&\, y_t - (\tilde{x}_t-x_t)^\intercal\,A(u_t)(\tilde{x}_t-x_t)\\ 
    =&\, \langle\tilde{\theta}_t,\tilde{x}_t\rangle - (\tilde{x}_t-x_t)^\intercal\,A(u_t)(\tilde{x}_t-x_t), \nonumber
\end{align}
where $A(u_t)\in\mathbb{R}^{n\times\,n}$ is a positive symmetric matrix, dependent on the agent's private type $u_t$, which expresses the cost for an agent to reveal features that are different than their true features. Neither the cost matrix $A(u_t)$ nor agent reward $y_t^{\text{agent}}$ are observed by the learner.

While the learner is interested in maximizing the long-term cumulative rewards --or equivalently treatment effects--  across all agents, the agents are self-interested individuals whose objective is to maximize their own expected reward $y_t^{\text{agent}}$, i.e.
\begin{equation}
    \label{eq:x-selection}
    \tilde{x}_t \in \argmax_{x_t'} y_t^{\text{agent}} = \argmax_{x_t'}\,\langle\tilde{\theta}_t,x_t'\rangle - (x_t'-x_t)^\intercal\,A(u_t)(x_t'-x_t)
\end{equation}

We can solve for $\tilde{x}_t$ in terms of $A(u_t), \tilde{\theta}_t$, and $x_t$ here by finding the inflection point of the gradient of the agent's objective function with respect to $\tilde{x}_t$, i.e.

\begin{align*}
    \nabla_{x_t}\,\langle\tilde{\theta}_t,\tilde{x}_t\rangle - (\tilde{x}_t-x_t)^\intercal\,A(u_t)(\tilde{x}_t-x_t)
    &= \tilde{\theta}_t - 2(\tilde{x}_t-x_t) = 0\\
    \Rightarrow \tilde{x}_t = \frac{[A(u_t)]^{-1}\tilde{\theta}_t}{2} + x_t.
\end{align*}


\xhdr{History}
The interaction between the planner and the agent $t$ is given by the tuple $(\tilde{\theta}_t, \tilde{x}_t, y_t)$. 
For each $t$, let $H_t$ denote the history from round 1 to $t$, that is the sequence of interactions between the social planner and first $t$ agents: $\left\{ (\tilde{\theta}_1, \tilde{x}_1, y_1), \ldots ,(\tilde{\theta}_t, \tilde{x}_t, y_t) \right\}$.


\textbf{Working}

==> pp.tex <==
\section{Performative prediction in our setting}\label{sec:pp}

Performative prediction methods perform repeated gradient descent \emph{without} taking into account $\vx_t$ and $y_t$'s explicit dependence on $\vtheta_t$. Because of this, their gradient (denoted by $\Delta_{PP}$) takes the form 

\begin{equation*}
    \boldsymbol \Delta_{PP} = \nabla_{\vtheta_t} f(\vtheta_t) = 2\mathbb{E}[(\widehat{y}_t - y_t)\vx_t].
\end{equation*}

This is in contrast to our gradient, $\Delta$, which takes the explicit dependence of $\vx_t$ and $y_t$ on $\vtheta_t$ into account.

\begin{equation*}
    \boldsymbol \Delta = \nabla_{\vtheta_t} f(\vtheta_t) = 2\mathbb{E}[(\widehat{y}_t - y_t)(\vx_t + W_tW_t^\top (\vtheta_t - \vtheta^*))].
\end{equation*}

We now show that the sign of $\boldsymbol \Delta$ and $\boldsymbol \Delta_{PP}$ can differ, using a simple 1D example. By writing $\vx_t$, $\hat y_t$, and $y_t$ in terms of $\vtheta_t$ and simplifying, we can see that for zero-mean $\vz_t$ and $g_t$,

\begin{equation*}
    \Delta_{PP} = 2\mathbb{E}[x_t^2](\theta_t - \theta^*) - \mathbb{E}[z_t g_t],
\end{equation*}
and 
\begin{equation*}
    \Delta = 2\mathbb{E}[x_t^2](\theta_t - \theta^*) - \mathbb{E}[z_t g_t] + W^4 \theta_t (\theta_t - \theta^*)^2.
\end{equation*}
Notice that if $\theta_t > 0$, $\theta^* > \theta_t$, $\mathbb{E}[z_t g_t] > 0$, and $W$ is large enough, then $\Delta > 0$ but $\Delta_{PP} < 0$.

==> prelims.tex <==

\subsection{Recommendations as Instruments}

We model the \dncomment{observed} reward $y_t$ and action $x_t$ in the presence of confounding variables that depend on the type $u_t$. In a standard bandits setting, without confounding variables, one would find \dncomment{the treatment effect} $\theta$ by taking the mean over sufficiently many observed rewards of each arm. However, because of the unknown confounding variable $g(u_t)$ that is correlated with $x_t$, such simple estimation does not work. Instead, we will use \textit{instrumental variable (IV) regression} to  estimate the exogenous treatment effect $\theta$. Note that each recommendation $z_t$ can be viewed an \textit{instrumental variable} because: (1) $z_t$ influences the selection $x_t$; and (2) $z_t$ is independent from the endogenous error term $g(u_t)$. Criterion (2) follows because planner chooses $z_t$ randomly independent of the type $u_t$. 



\iffalse 
IV regression estimates the treatment effect when the explanatory variable is correlated with the error term. The reward model in equation~\eqref{eq:reward-model} follows the form of a model for treatment effect: the treatment $x_t$, the exogenous treatment effect $\theta$, and the error term $g(u_t) + \epsilon_t$ determine the response variable $y_t$. Both the treatment $x_t$ and the reward $y_t$ are correlated with the endogenous error term $g(u_t)$.
\fi


Our mechanism periodically solves the following IV regression problem:
given a set of $n$ observations $\{(x_i, y_i, z_i)\}_{i=1}^n$, find an accurate estimator $\hat \theta_n$ of $\theta$. To derive the estimator, we will rewrite the selection and reward functions in~\eqref{eq:reward-model} and \eqref{eq:two-arm-general-selection-function} as a linear relationship between $x_i$, $y_i$ and $z_i$. Then
\begin{align}
    y_i &= \theta x_i + g(u_i) + \eps_i \label{eq:reward-iv-model}\\
    x_i &= \gamma_1 z_i + \gamma_0(1-z_i) + \eta_i \nonumber\\
    &= \gamma z_i + \gamma_0 + \eta_i \label{eq:treatment-iv-model}
\end{align}
 where $\eta_i=\E_\cU[x \mid z_i] - x_i$ and $\gamma_1=\Prob_{\cU}[x_i=1 \mid z_i=1]$ and $\gamma_0=\Prob_{\cU}[x_i=1 \mid z_i=0]$ make up the \emph{compliance coefficient} $\gamma$, which is given by:
 \begin{equation}
    \label{eq:compliance-coefficient}
     \gamma=\gamma_1-\gamma_0=\Prob_{\cU}[x_i=1 \mid z_i=1]-\Prob_{\cU}[x_i=1 \mid z_i=0]
 \end{equation}

Let the operator $\bar{\cdot}$ denote the mean, such that $\bar{y}:=\frac{1}{n}\sum_{i=1}^n y_i$ and $\bar{g}:=\frac{1}{n}\sum_{i=1}^n g(u_i)$, etc. Then, the average observed reward is 
\begin{align*}
    \bar{y} &= \beta\bar{z} + \theta\gamma_0 + \theta\bar{\eta} + \bar{g} + \bar{\epsilon}
\end{align*}
Thus, the centered reward and treatment choice at round $i$ are given as:
\begin{equation}
    \begin{cases}
    \label{eq:centered-reward-treatment-choice}
    y_i - \bar{y}_i = \beta(z_i-\bar{z}) + \theta(\eta_i-\bar{\eta}) + g(u_i)-\bar{g} + \epsilon_i-\bar{\epsilon}\\
    x_i - \bar{x}_i = \gamma(z_i-\bar{z}) + \eta_i-\bar{\eta}
    \end{cases}
\end{equation}


\textbf{Instrumental Variable Estimator.} Using these formulations of the centered reward $y_i-\bar{y}$ and treatment choice $x_i-\bar{x}$, we form the estimate $\hat{\theta}_n$ via \textit{Instrumental Variable (IV) regression}. We first form empirical estimates $\hat{\gamma}_n$ and $\hat{\beta}_n$ by regressing the centered treatment choice $x_i-\bar{x}$ and the centered reward $y_i-\bar{y}$ over the centered recommendation $z_i-\bar{z}$, respectively. These estimates are formed over $n$ samples $\{x_i,z_i,y_i\}_{i=1}^n$ as such:
\begin{equation}
    \hat{\beta}_n := \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2} \hspace{1cm}\text{and}\hspace{1cm} \hat{\gamma}_n := \frac{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2}
    \label{eq:beta-gamma-hat}
\end{equation}
Second, we take their quotient as the predicted treatment effect $\hat{\theta}_n$, i.e. 
\begin{align}
    \hat{\theta}_n &= \frac{\hat{\beta}_n}{\hat{\gamma}_n}\\
    &= \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (z_i -\bar{z})^2} \frac{\sum_{i=1}^n (z_i -\bar{z})^2}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})} \nonumber\\
    &= \frac{\sum_{i=1}^n (y_i - \bar{y})(z_i - \bar{z})}{\sum_{i=1}^n (x_i - \bar{x})(z_i - \bar{z})}
\end{align}

We provide a finite-sample \textit{approximation bound} on $\hat{\theta}_n$, which may be of independent interest.

\begin{restatable}[Treatment effect approximation bound]{theorem}{treatmentapproximationbound}\label{thm:treatment-approximation-bound}
        Given a sample set $(z_i, x_i, y_i)_n$, which contains $n$ samples of instrument $z$, treatment $x$, and reward $y$, we bound the difference between the true treatment effect $\theta$ and the predicted treatment effect $\hat{\theta}_n$ derived via IV regression over $(z_i, x_i, y_i)_n$. Let $\Upsilon$ be a upper bound on the confounding term $g(u_i)$. For some confidence $\delta>0$, with probability at least $1 - \delta$:
\[\left|\hat{\theta}_n-\theta\right| \leq \frac{\left(2\sigma_{\eps}+2\Upsilon\right)\sqrt{2n\log(5/\delta)}}{\left|\sum_{i=1}^n(x_i-\bar{x})(z_i-\bar{z})\right|}\]
\end{restatable}

\begin{proof}
    See \cref{sec:approximation-bound-proof} for a proof.
\end{proof}


==> related-works.tex <==
\section{Related Work}

\subsection{Comparison with \cite{shavit2020strategic}}

The setting most similar to ours is that of \cite{shavit2020strategic}. They consider a strategic classification setting in which an agent's outcome is a linear function of features --some observable and some not (see \Cref{fig:shavit-model-dag} for a graphical representation of their model). While they assume that an agent's hidden attributes can be modified strategically, we choose to model the agent as having an unmodifiable private \emph{type}. Both of these assumptions are reasonable, and some domains may be better described by one model than the other. For example, the model of \cite{shavit2020strategic} may be useful in a setting such as car insurance pricing, where some unobservable factors which lead to safe driving are modifiable. On the other hand, settings like our college admissions example in which the unobservable factors which contribute to college success (i.e. socioeconomic status, lack of resources, etc., captured in $g_t$) are not easily modifiable.
\hhcomment{The preceeding claim does not appear to be true. In our setting, action/effort is modifiable and unobservable.}

One benefit of our setting is that we are able to use $\vtheta_t$ as a valid instrument to recover the true relationship $\vtheta^*$ between observable features and outcomes. This is generally not possible in the model of \cite{shavit2020strategic}, since $\vtheta_t$ violates the backdoor criterion as long as there exists any hidden features $\mathbf{h}_t$ and is therefore not a valid instrument. Another difference between our setting and theirs is that we allow for a heterogeneous population of agents, while they do not. Specifically, they assume that each agent's mapping from actions to features is the same, while our model is capable of handling mappings which vary from agent-to-agent.

A natural question is whether or not there exists a general model which captures the setting of both \cite{shavit2020strategic} and ours. We provide such a model in \Cref{fig:general-model-dag}. In this setting, an agent has both observable and unobservable features, both of which are affected by the assessment rule $\vtheta_t$ deployed and the agent's private type $u_t$. However, much like the setting of \cite{shavit2020strategic}, $\vtheta_t$ violates the backdoor criterion, so it cannot be used as a valid instrument in order to recover the true relationship between observable features and outcomes. Moreover, the following toy example illustrates that \emph{no} form of true parameter recovery can be performed when an agent's unobservable features are modifiable.

\begin{figure}
    \begin{subfigure}[t]{0.49\textwidth}
         \centering
             \begin{tikzpicture}[node distance={22mm}, thick, main/.style = {draw, circle}] 
             \node[draw,circle,fill=lightgray] (1) {$\vtheta_t$}; 
             \node[draw,circle,fill=lightgray] (2) [right of=1,yshift=0.65cm] {$\vx_t$}; 
             \node[node distance={15mm}, thick,draw,circle] (3) [below of=2] {$\mathbf{h}_t$};
             \node[draw,circle,fill=lightgray,,yshift=-0.65cm] (4) [right of=2] {$y_t$};
             \draw[->] (1) -- node[above left,xshift=0.35cm] {$\va_t$, $W_t$} (2);
             \draw[->] (1) -- node[below left,xshift=0.35cm] {$\va_t$, $W_t$} (3);
             %\draw[->] (2) -- node[left] {$z_t$} (3);
             % \draw (1) to [out=180,in=270,looseness=5] (1);
             \draw[->] (3) -- node[below right=-0.15cm] {$\vtheta^*$} (4);
             \draw[->] (2) -- node[above] {$\vtheta^*$} (4);
             \end{tikzpicture} 
         \caption{Graphical model of \cite{shavit2020strategic}. Observable features $\vx_t$ (e.g. the type of car a person drives) and unobservable features $\mathbf{h}_t$ (e.g. how defensive of a diver someone is) are affected by $\vtheta_t$ through action $\va_t$ (e.g. buying a new car) and common action conversion matrix $W$ (representing, in part, the cost to a person of buying a new car). Outcome $y_t$ (in this example, the person's chance of getting in an accident) is affected by $\vx_t$ and $\mathbf{h}_t$ through the true causal relationship $\vtheta_t$. Note that causal parameter recovery is not possible in this setting unless all features are observable.}
         \label{fig:shavit-model-dag}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.49\textwidth}
         \centering
             \begin{tikzpicture}[node distance={25mm}, thick, main/.style = {draw, circle}] 
             \node[draw,circle,fill=lightgray] (1) {$\vtheta_t$};
             \node[draw,circle,fill=lightgray] (2) [right of=1] {$\vx_t$}; 
             \node[node distance={20mm},draw,circle,fill=lightgray,yshift=-1.2cm] (3) [right of=2] {$y_t$};
             \node[main] (4) [below of=1] {$u_t$};
             \node[main] (5) [right of=4] {$\mathbf{h}_t$};
             \draw[->] (1) -- node[above] {$\va_t$} (2);
             \draw[->] (2) -- node[above] {$\vtheta^*$} (3);
             \draw[->] (1) -- node[above right,yshift=0.5cm,xshift=-0.55cm] {$\va_t$} (5);
             \draw[->] (4) -- node[above,yshift=-.7cm,xshift=-1cm] {$\vz_t,W_t$} (2);
             \draw[->] (5) -- node[below] {$\vtheta^*$} (3);
             \draw[->] (4) edge[bend right=2cm] node [below right]{$g_t$} (3);
             \draw[->] (4) -- node[above] {$\vz_t,W_t$} (5);
             \end{tikzpicture} 
         \caption{Graphical model which captures both our setting and that of \cite{shavit2020strategic}. In this setting, observable features $\vx_t$ \emph{and} unobservable features $\mathbf{h}_t$ are affected by $\vtheta_t$ through action $\va_t$. The agent's private type $u_t$ affects $\vx_t$ and $\mathbf{h}_t$ through initial feature values $\vz_t$ and action conversion matrix $W_t$. The agent's outcome $y_t$ depends on $\vx_t$ and $\mathbf{h}_t$ through the causal relationship $\vtheta^*$ and $u_t$ through confounding term $g_t$. Note that much like the setting of \cite{shavit2020strategic}, causal parameter recovery is not possible in this setting unless all features are observable.}
         \label{fig:general-model-dag}
    \end{subfigure}
\end{figure}

\begin{example}
    Consider the one-dimensional setting 
    \begin{equation*}
        y_t = \theta^*x_t + \beta^* h_t, 
    \end{equation*}
    
    where $x_t$ is an agent's observable, modifiable feature and $h_t$ is an unobservable, modifiable feature. If the relationship between $x_t$ and $h_t$ is unknown, then it is generally impossible to recover the true relationship between $x_t$, $h_t$, and outcome $y_t$. To see this, consider the setting where $h_t$ and $x_t$ are highly correlated. In the extreme case, take $h_t = x_t, \; \forall t$. (Note we use equality to indicate identical feature values, not a causal relationship.) In this setting, the models $\theta^* = 1$, $\beta^* = 1$ and $\theta^* = 2$, $\beta^* = 0$ produce the same outcome $y_t$ for all $x \in \mathbb{R}$, making it impossible to distinguish between the two models, even in the limit of infinite data.
\end{example}

\subsection{Comparison with Performative Prediction}
A recent line of work (\cite{perdomo2020performative, mendler2020stochastic, miller2021outside}) examines the use of repeated gradient descent in strategic learning setting and finds that under certain conditions on the predictive risk function, performative prediction methods converge to \emph{performatively stable} or \emph{performatively optimal} points. Performatively optimal points are analogous to global minima in our setting, but there is no direct comparison between performatively stable points and local minima in our setting. Our methods differ from this line of work because we take $\vx_t$, $y_t$, and $\widehat{y}_t$'s \emph{direct dependence} on the assessment rule $\vtheta_t$ into account when calculating the gradient of the risk function, whereas these performative prediction models do not. Because of this, we can guarantee convergence to local minima of the predictive risk function, whereas this is generally not guaranteed under the performative prediction framework. For a more detailed analysis of performative prediction repeated gradient descent in our setting, see Appendix \ref{sec:pp}.
